A Closer Look at the Security Risks in the Rust Ecosystem

Rust is an emerging programming language designed for the development of systems software. To facilitate the reuse of Rust code, crates.io, as a central package registry of the Rust ecosystem, hosts thousands of third-party Rust packages. The openness of crates.io enables the growth of the Rust ecosystem but comes with security risks by severe security advisories. Although Rust guarantees a software program to be safe via programming language features and strict compile-time checking, the unsafe keyword in Rust allows developers to bypass compiler safety checks for certain regions of code. Prior studies empirically investigate the memory safety and concurrency bugs in the Rust ecosystem, as well as the usage of unsafe keywords in practice. Nonetheless, the literature lacks a systematic investigation of the security risks in the Rust ecosystem. In this paper, we perform a comprehensive investigation into the security risks present in the Rust ecosystem, asking ``what are the characteristics of the vulnerabilities, what are the characteristics of the vulnerable packages, and how are the vulnerabilities fixed in practice?''. To facilitate the study, we first compile a dataset of 433 vulnerabilities, 300 vulnerable code repositories, and 218 vulnerability fix commits in the Rust ecosystem, spanning over 7 years. With the dataset, we characterize the types, life spans, and evolution of the disclosed vulnerabilities. We then characterize the popularity, categorization, and vulnerability density of the vulnerable Rust packages, as well as their versions and code regions affected by the disclosed vulnerabilities. Finally, we characterize the complexity of vulnerability fixes and localities of corresponding code changes, and inspect how practitioners fix vulnerabilities in Rust packages with various localities.

==> sections/RQ.tex <==
We aim to gain insights into the evolution and security risks of the Rust ecosystem. To achieve this goal, our study is structured around four research questions as follows: 

%\textbf{RQ1: Library Usage Analysis.} How many Rust libraries over time?
% \noindent\textbf{RQ1: What are the characteristics of libraries in the Rust ecosystem?}

\noindent\textbf{RQ1: How does the Rust ecosystem evolve over time?}

%\zy{[TWO LAYERS: without categories; with categories] Total crates; Evolution from two aspects: (a) growth in the number of packages (added/updated to crates.io) (b) evolution of package popularity (downloads)}
% We started analyzing how the Rust ecosystem evolves over time. We measured evolution in three aspects: the number of packages over time, the number of packages newly created every month, and the downloads of packages over time. Such an analysis can help researchers understand the popularity of the Rust ecosystem.
We start with an investigation of how the Rust ecosystem evolves over time, to understand the ecosystem per se. Specifically, we measure the evolution of the Rust ecosystem from two aspects: the evolution of the number of packages and the evolution of package popularity. %This could help contributors to sustain the level and number of high-quality contributions. 
The understanding of ecosystem evolution could help gain insights into sustaining high-quality contributions in software ecosystems. 
%\todo{[Jun 22] @xiaoye, could you please add 1 to 2 sentences to describe the motivation of this RQ? (consider referring to previous ecosystem papers:-)}


%\textbf{RQ2: Library Vulnerability Analysis.} How many vulnerabilities are in Rust libraries? How are they distributed?
% \noindent\textbf{RQ2: What categories of vulnerabilities appear in Rust libraries?}

\noindent\textbf{RQ2: What are the characteristics of vulnerabilities in the Rust ecosystem?}
%\zy{[May 18] what are they (categories)? where are they? e.g., they tend to be from the most popular crates; or a particular category, some categories of crates are more prone to others? -- we could connect RQ2 with RQ1 from here:-)}
%Second, we studied the characteristics of vulnerabilities in the Rust ecosystem. We focused on three aspects: (1) type of vulnerabilities; (2) vulnerability evolution; (3) vulnerability locality. We investigated what are the categories of vulnerabilities, where the vulnerabilities (e.g., they tend to be in \textcolor{ao(english)}{\tt unsafe} code, some categories of crates are more prone to others). This helped to answer a key question "Is Unsafe really unsafe?". If yes, then most vulnerabilities can be avoided by writing the code in Safe Rust. If not, then the vulnerabilities lie within Rust code itself and may be necessary for achieving the desired safeness with careful logic analysis or rust language itself. The motivation of RQ2 is to understand security risks in the Rust ecosystem.

We focus on two aspects to characterize the vulnerabilities in the Rust ecosystem: (1) type of vulnerabilities, and (2) vulnerability evolution. Previous studies~\cite{pldi2020,tosem2021} only focus on  memory safety and concurrency bugs but do not consider other types of vulnerabilities in the Rust ecosystem. %We would like to provide insights into vulnerabilities in the Rust ecosystem and build a systematic view of vulnerabilities in the Rust ecosystem.
We would like to build a systematic view of a variety of  vulnerabilities in the Rust ecosystem.
%
% \todo{[Jun 22] @xiaoye, could you please refer to 1-2 papers, stating that our investigation about vulnerabilities here is important:-)}
%

\noindent\textbf{RQ3: What are the characteristics of the vulnerable packages in the Rust ecosystem?}

Packages are reused in software ecosystems to minimize redundant development efforts, introducing potential risks that propagate through multiple levels of dependencies in packages~\cite{kikas2017structure, zimmermann2019small}. A prior study~\cite{icse2020evan} investigates the usage of unsafe code in  Rust packages. However, it remains unclear whether unsafe Rust code undermines the security of Rust packages in practice, and whether unsafe Rust code introduces more vulnerabilities compared with safe Rust code. % but does not bridge the gap between unsafe code and vulnerabilities. 
%
%\todo{[Jul 30] Please update the sentence above, by clarifying what is not done in~\cite{icse2020evan}; and update the sentence below, by clarifying what is not done in~\cite{icse2020evan} will be investigated in our work :-) } \xy{[Aug 1]Updated.}
%
Thus, we would like to investigate the locality of vulnerabilities in the Rust packages, and further analyze the relations between unsafe code and vulnerabilities. %--whether the vulnerable code tends to locate in \textcolor{ao(english)}{\tt unsafe} code. 
% To understand the security risks of the Rust ecosystem, we are curious about how vulnerabilities affect Rust packages and what package categories are more prone to vulnerabilities. We also investigate the locality of vulnerable code in the Rust packages, including whether the vulnerable code tends to locate in \textcolor{ao(english)}{\tt unsafe} code. 
%
%Packages could be reused in OSS ecosystems to minimize redundant effort, which could also introduce risks and propagate through multiple levels of dependencies\cite{kikas2017structure, zimmermann2019small}. Therefore, identifying the characteristics of the vulnerable packages is important. Furthermore, Evans\cite{icse2020evan} investigates the usage of unsafe code in the Rust ecosystem but does not bridge the gap between unsafe code and vulnerabilities. 
%Furthermore, Evans\cite{icse2020evan} investigates the usage of unsafe code in the Rust ecosystem but does not bridge the gap between unsafe code and vulnerabilities. 
%
%\todo{[Jun 22] @xiaoye, could you please refer to two to three papers (1-2 about vul effects package,  1-2 about unsafe Rust), stating that our investigation here is important:-)}
%
% The answer to this research question could help to answer the question ``is \textcolor{ao(english)}{\tt unsafe} really unsafe?''. If the answer is yes, most of the vulnerabilities may be prevented by writing code in safe Rust. If the answer is no, to achieve security requirements, it is necessary to conduct an in-depth analysis when writing code in safe Rust or enhance the security of the Rust language. 
%
%Besides, we are curious about how vulnerabilities affect Rust packages and what package categories are more prone to vulnerabilities. 
%
%The answering question could provide insights into the differences in security risks across package categories in the Rust ecosystem.

% \textbf{RQ3:  Library Risk Analysis.} Whether vulnerabilities of rust libraries are caused by unsafe code in rust libraries?

% \noindent\textbf{RQ3: Are vulnerabilities in Rust libraries introduced by \textcolor{ao(english)}{\tt unsafe} Rust?}

%\noindent\textbf{RQ3: How are vulnerabilities in the Rust ecosystem introduced and fixed in practice?}
\noindent\textbf{RQ4: How are vulnerabilities in the Rust ecosystem fixed in practice?}

%After studying vulnerability in the Rust ecosystem, we moved toward the understanding of the characteristics of vulnerability fixes. We firstly focused on the fix commit locality, e.i., where the fixing code locates. Next, we analyze how programmers fix vulnerabilities, e.g., whether they remove unsafe code to fix the vulnerabilities. Besides, we analyzed fix patterns of vulnerabilities.
In this research question, we move forward to characterize Rust vulnerability fixes in practice. The understanding of vulnerability fixes provides insights to practitioners when they encounter emergent security concerns~\cite{CCS2017Patches}. 
%
We wonder where code changes of vulnerability fix commits locate, and how developers fix Rust vulnerabilities with different localities in practice, e.g., whether developers tend to remove unsafe functions to fix vulnerabilities. 
%
We expect that the answer to this question could be helpful for practitioners to fix Rust vulnerabilities with respect to their types and localities.
%
%Practitioners could gain insights from the fix patterns in practice when they encounter emergent security concerns~\cite{CCS2017Patches}. The investigation of vulnerability fixes in the Rust ecosystem could provide practitioners with some hints on how to fix a Rust vulnerability in terms of its locality.  

%
%\todo{[Jun 22] @xiaoye, could you please refer to one paper or two, saying our motivation to investigate vul fixes?}


==> sections/discussion_old.tex <==
We now summarize our main results, discuss their implications,  and highlight the avenues for future research.

% \xy{[Aug 1] New.}
% \todo{[Aug 4] @Xiaoye, please split as needed and conclude the comparison results of the below paragraph with one sentence to replace the title.}
% \noindent\textbf{Rust is an emerging and growing software ecosystem.}
% We would compare our findings in the Rust ecosystem with npm, PyPI, and Maven ecosystem. Then we delve into some of the reasons ecosystems exhibit some similar characteristics as well as explanations about the divergent findings. npm ecosystem is created in 2009 and has grown steadily to feature over 230, 000 packages in January, 2016~\cite{kikas2017structure,msr2016npm}. PyPI ecosystem grows exponentially over the period 2006 to 2018, as it sustained around 40\% growth rates of new packages over the 13 year~\cite{Bommarito2018PyPI}. On 17 January 2022, PyPI hosts more than 350,000 Python packages. The Maven ecosystem also grows exponentially from 2004 to 2017 and slows down from 2018~\cite{mvn2022repo}. It indexes more than 29,000,000 packages in Aug 2022. Our results show that Rust is an emerging ecosystem since its creation in 2014. Over the last seven years (2014 to 2021), the ecosystem has rapidly grown and currently hosts over 80,000 packages. We observed that Rust is still a small and emerging ecosystem compared to other ecosystems and has room for growth. The rust ecosystem is still in exponential growth and has no sign of stagnation compared to the Maven ecosystem. Our findings show that the popular categories in Rust are command line utilities and development tools. The most popular category in PyPI is software development~\cite{Bommarito2018PyPI}. Popular categories in Java are testing frameworks and android packages. We observe that utilities and development tools gain popularity in the growing ecosystems and mature ecosystems pay more attention to application-related packages. The possible reason for the switch might be the basic tools and utilities in the mature ecosystem are well-developed.

\noindent\textbf{Rust is an active and growing software ecosystem at its early stage.}
A comparison between our findings regarding the Rust ecosystem with those in previous studies, e.g., the npm, PyPI, and Java ecosystems, suggests the stage of Rust ecosystem in its evolution. 
%

%In terms of ecosystem evolution, 
\hl{The npm ecosystem, created in 2009, has grown steadily to feature over 2,210,000 packages in December 2022}\footnote{\url{http://www.modulecounts.com/}}. The PyPI ecosystem grows exponentially over the period from 2006 to 2018, sustaining around a 40\% growth rate of new packages ~\cite{Bommarito2018PyPI}; PyPI hosts more than 350,000 Python packages up to January 2022. 
%
Similar to the PyPI ecosystem, the Maven ecosystem grows exponentially from 2004 to 2017, but the growth slows down since 2018~\cite{mvn2022repo}; Maven indexes more than 29,000,000 \hl{artifacts} in August 2022. 
%
As our results in the preliminary investigation indicate, the Rust ecosystem, created in 2014, has been experiencing exponential growth over the last seven years (from 2014 to 2021) and has no sign of stagnation. The Rust ecosystem hosts over 80,000 packages until recently. %\hl{Maven and npm ecosystem have large package size (over 2 millions) and may not comparable with Rust ecosystem in number of packages alone, but the trend of package growth could give us some insights on the evolution of Rust ecosystem.}
%
%
%The relatively smaller number of packages in the Rust ecosystem and faster growth compared to other ecosystems indicates the Rust ecosystem still has growth potential. 
\hl{The Maven and npm ecosystems, as mature software ecosystems, have over 2 millions packages, which is significantly greater than the number of packages in the Rust ecosystem. The comparison of growth in the numbers of packages across ecosystems give insight into the evolution stage of the Rust ecosystem. Specifically, compared to other ecosystems, the relatively smaller number of packages and faster growth indicates that the Rust ecosystem is an active and growing software ecosystem at its early stage.}
% \hl{Interestingly, we also found that there was a dip in Rust activity in mid-late 2020, which may be caused by Mozilla lay-offs\footnote{\url{https://blog.rust-lang.org/2020/08/18/laying-the-foundation-for-rusts-future.html}} and we left this as a future work for more detailed and precise analysis.}
\hl{Interestingly, we found that the increasing number of packages per month experiences a sharp decline in the Rust ecosystem in mid-late 2020, which may be caused by Mozilla lay-offs\footnote{\url{https://blog.rust-lang.org/2020/08/18/laying-the-foundation-for-rusts-future.html}}. Future work could systematically investigate the factors that influence the activities in the Rust ecosystem.}
%

%In terms of popular package categories, 
Utilities and development tools tend to gain popularity in growing software ecosystems such as Rust and PyPI. Specifically, the top 2 most popular categories of Rust packages are \emph{no standard library} and \emph{development tools}; the most popular category in PyPI is \emph{software development}~\cite{Bommarito2018PyPI}. \hl{Although Python dose not have unsafe memory features, memory and concurrency related vulnerabilities exist in the packages of the PyPI ecosystems.} As for mature software ecosystems like Java, practitioners pay more attention to application-related packages, e.g., Android. 
%
The difference in package popularity between growing and mature software ecosystems might be due to that the tools and utilities have been well developed in mature software ecosystems. \hl{Future work could also investigate the data collection and analysis of the sub-categories of packages in the \emph{no standard library} category, which is the most popular category of packages in the Rust ecosystem.}


% \noindent\textbf{The awareness of vulnerabilities in Rust is increasing.}
% Studies on PyPI and npm ecosystems found that the number of newly discovered vulnerabilities is growing over time~\cite{Bommarito2018PyPI}. Our work also shows that discovered vulnerabilities in Rust are growing and keeping up with the growth of the ecosystem. The increase in the number of reported vulnerabilities in different ecosystems is a result of coordinated efforts in increasing awareness of vulnerabilities and continuous process testing packages to identify the vulnerabilities before they can be exploited. However, the most common type of vulnerability differs. Memory safety and concurrency issues take two-thirds of vulnerabilities in the Rust ecosystem as our work shows, while Cross-Site-Scripting (XSS) is the most common type of vulnerability in both PyPI and npm ecosystem~\cite{Bommarito2018PyPI}. The possible reason for the difference would be that Rust is a language for system development and focuses on solving memory safety problems, but npm and PyPI are more popular in web applications.

\noindent\textbf{The awareness of vulnerabilities in the Rust ecosystem is increasing.}
In the Rust ecosystem, the number of vulnerabilities reported per 1,000 packages grows from one in 2017 to almost ten in 2022 (RQ1).
%
Previous studies also found that the number of newly reported vulnerabilities is growing over time in the PyPI and npm ecosystems~\cite{Bommarito2018PyPI}. 
%
The increase in the number of reported vulnerabilities in a software ecosystem can attribute to the coordinated efforts in increasing awareness of vulnerabilities and continuous process testing packages to identify the vulnerabilities before they can be exploited. 
%


Interestingly, the most common type of vulnerability differs across various software ecosystems. Memory safety and concurrency issues account for two-thirds of the vulnerabilities in the Rust ecosystem (RQ1), while cross-site scripting (XSS) is the most common type of vulnerability in both PyPI and npm ecosystems~\cite{Bommarito2018PyPI}. 
%
The frequent occurrence of memory safety and concurrency issues may be due to that Rust is a language for systems software development; Systems software developers tend to manipulate memory and threads in their code more frequently compared with developers of other types of software. %
The frequent occurrence of XSS in the PyPI and npm ecosystems may be because practitioners tend to use npm and PyPI packages for the development of web applications.


%\noindent\textbf{There is a dire need for more efforts in developing popular packages.}
%Our findings show that some package categories with high downloads did not increase significantly in the number of packages (RQ1). Specifically, the \emph{Algorithms} and \emph{Asynchronous} categories rank in the top 5 in terms of package downloads but rank out of the top 10 in terms of package number. And the \emph{memory management} and \emph{concurrency} categories grow exponentially in terms of downloads, but grow linearly in terms of package numbers. The results imply that some popular package categories which have gained wide attention do not have enough resources available to users, resulting in limited choices for users in these categories of packages. For the Rust community, more effort should be devoted to these popular categories with high user attention, and more packages should be developed for users to choose from. In future work, researchers could study how to perceive the trend of the popularity of package categories in advance, to provide some reference for practitioners.

%Some popular category of packages has relatively fewer choices for users. The Rust community should put more effort into developing packages of those categories.

%\noindent\textbf{Patches are not available or broken. Thus, we need tools to identify security packages in the Rust ecosystem.} (CCS 2017 - security patch)

%"We identified a total of 338 vulnerable packages, accounting for 0.40\% of packages in the Rust ecosystem. Note that 120 out of 338 vulnerable packages remain unpatched."


%\noindent\textbf{Safe code is more vulnerable to vulnerabilities than unsafe code.}
% \noindent\textbf{Safe code is more prone to vulnerabilities than unsafe code in the Rust ecosystem.} Safe functions account for 85\% of the functions in the code repositories of vulnerable packages affected by reported vulnerabilities (RQ3). Note that 26.9\% of the safe functions affected include unsafe blocks in their function bodies (RQ3). At the same time, we also studied the fix patterns of vulnerabilities in Rust, vulnerability fixes in the Rust ecosystem involve an average of 49 lines of code added and 26 lines of code deleted, and reside in 4.15 safe functions, 0.65 unsafe functions, and 0.92 unsafe blocks on average (RQ4). Our research results show that unsafe functions are not really ``unsafe'', unsafe code is not more prone to vulnerabilities. On the contrary, most of the vulnerabilities appear in safe functions, and unsafe code is not the main reason for the increase in vulnerabilities. Developers should focus more on how to ensure the reliability of safe code. In addition, when fixing vulnerabilities, developers are more inclined to modify safe and unsafe code, rather than directly remove unsafe code. This indicates that removing unsafe code is not a good strategy to secure Rust software systems. Practitioners should comprehensively consider the issues in safe and unsafe code, and take a variety of measures to protect Rust software systems.
% \noindent\textbf{Safe functions tends to be more prone to vulnerabilities than unsafe functions in the Rust ecosystem.} 
%
% Meanwhile, vulnerability fixes in the Rust ecosystem reside in 3.85 safe functions, 0.16 unsafe functions, and 1.49 unsafe blocks on average (RQ3). 
%
% A recent study~\cite{icse2020evan} reveals that practitioners use the unsafe keyword in 29\% of Rust libraries. 
%
% The relatively higher occurrence of vulnerabilities in safe code indicates that safe code tends to be more prone to vulnerabilities than unsafe code in the Rust ecosystem --  ``unsafe code is not really unsafe''. 
%
%Practitioners could put forth more effort into ensuring the security of safe Rust code, e.g., via compiler checks. 
%
% The results provide insights for practitioners to fix potential security issues in Rust code repositories.
%
\noindent\textbf{\hl{Most of vulnerabilities involve safe functions.}} 95\% of the functions affected by reported vulnerabilities are safe functions (RQ2).
%
Among the safe functions affected by vulnerabilities, 41.5\% includes unsafe blocks in their function body (RQ2). The high occurrence of vulnerabilities in safe functions indicates that vulnerabilities would not strictly restricted inside the unsafe code. 
%
 In terms of fixing vulnerabilities, prior study~\cite{CCS2017Patches} reported that the median security commit diff involved 7 LOC. Our investigation of the Rust ecosystem revealed that the median fix commit diff includes a median of 14 added lines, 4 deleted lines, indicating that the fixes in Rust are more complex. Moreover, the study found that 59\% of security changes were located in a single function~\cite{CCS2017Patches}, while our investigation showed that the median fix commit involves one safe function (with a mean of 3.85), suggesting that the fixes in Rust are less localized in the Rust ecosystem.
 % 
 In addition, developers tended to modify safe and unsafe code, rather than directly remove unsafe code in a vulnerable code repository (RQ3). This finding aligns with previous research that indicates developers typically update files rather than creating or deleting them~\cite{CCS2017Patches}.
%
The vulnerability fixing pattern indicates that removing unsafe code might not be a common measure for practitioners to secure Rust software systems in practice. 
%
The results also suggest a comprehensive consideration of both safe and unsafe code for fixing vulnerabilities in the Rust ecosystem.

\noindent\textbf{\hl{Vulnerable code in vulnerable packages involves more unsafe functions and unsafe blocks.}} Recent studies report that practitioners use the unsafe keyword in 29.4\% Rust libraries~\cite{icse2020evan}; unsafe functions account for 4.1\% of the functions in Rust packages~\cite{unsafeblog}; and 13.8\% safe functions have unsafe blocks in their body~\cite{unsafeblog}. \hl{The findings are comparable to the results in RQ2: unsafe functions account for 2.4\% of the functions in vulnerable Rust packages; 12.1\% of the safe functions have unsafe blocks in their body. In contrast, we observed that vulnerable code involves more unsafe functions and unsafe  blocks in RQ2. Specifically, unsafe functions account for 4.3\% of the functions affected by reported vulnerabilities; Meanwhile, 41.5\% safe functions have unsafe blocks in their body. The  observation implies that unsafe code tends to be more prone to vulnerabilities than safe code in the Rust ecosystem – “unsafe code is somewhat unsafe”. Thus, practitioners could put forth more effort into ensuring the security of unsafe Rust code.}

%A recent study~\cite{icse2020evan} reveals that practitioners use the unsafe keyword in 29.4\% of Rust libraries. Ozdemir~\cite{unsafeblog} shows that 4.1\% of functions in the Rust ecosystem are unsafe functions and at most 13.8\% safe functions have unsafe blocks in their body. 
%2.4\% of functions in the vulnerable packages are unsafe functions and 12.1\% safe functions have unsafe blocks in their body (RQ2). The difference between Rust ecosystem and vulnerable packages is not significant. 

%In contrast, as for vulnerable code in the repositories of vulnerable Rust packages, unsafe functions account for 4.3\% of the functions affected by reported vulnerabilities in the code repositories of vulnerable Rust packages and 41.5\% safe functions have unsafe blocks in their body(RQ2). The relatively higher occurrence of vulnerabilities in unsafe code indicates that unsafe code tends to be more prone to vulnerabilities than unsafe code in the Rust ecosystem – “unsafe code is somewhat unsafe”. Practitioners could put forth more effort into ensuring the security of unsafe Rust code, e.g., via compiler checks. 

% Besides, vulnerabilities have large chance residing in safe code considered to vulnerability types of \emph{tainted input} and \emph{resource management} (RQ2). Practitioners should also pay more attention to safe code when dealing with user input, directory path and etc. %Unsafe code tends to be more prone to vulnerabilities. If so, tools to protect unsafe code are important; otherwise, practitioners should take a variety of measures to secure Rust software systems. (ICSE 2020 Evans, PLDI 2020)


%\noident\textbf{Memory vulnerabilities.}
%TOSEM 2021


% \noindent\textbf{Differences exist in locality and fixes across various types of Rust vulnerabilities.}
% Different types of vulnerabilities have significant differences in vulnerability locality. For example, the \emph{memory access} vulnerabilities tend to mainly occur in safe functions, and the \emph{synchronization} vulnerabilities tend to locate in unsafe functions and unsafe blocks (RQ3). Therefore, for different types of vulnerabilities, practitioners can focus on different kinds of code when locating vulnerabilities. In addition, when fixing vulnerabilities, the number of safe functions involved in \emph{memory access} vulnerabilities is more than that involved in other vulnerability fixes (RQ4). Therefore, in future work, researchers could study different automated vulnerability fixing methods according to the differences in the introduction location, fix location, and fix pattern of different vulnerability types.
% \noindent\textbf{Differences exist in the locality of vulnerable code and fixes across various types of Rust vulnerabilities.}
% We observe difference exists in the locality of vulnerable code across various types of vulnerabilities (RQ2). For instance, the \emph{memory access} vulnerabilities tend to reside in unsafe blocks inside safe functions; the \emph{synchronization} vulnerabilities tend to locate in unsafe traits. The difference in vulnerability localities suggests that practitioners can focus on different code regions when localizing different types of vulnerabilities to save time and effort. 
%
% We also observe that fixing \emph{memory access} vulnerabilities tend to involve more safe functions compared with other types of vulnerabilities (RQ4). Future work could take into account the types of Rust vulnerabilities for the design of effective Rust program repair tools.

% \noindent\textbf{Rust vulnerability classification.}
% Among the 776 vulnerabilities we collected, 164 vulnerabilities have not been categorized (RQ2). This indicates that there are still a large number of vulnerabilities in the software repository that have not been assigned to the corresponding categories, which may affect the location and repair process of these vulnerabilities. Researchers could provide some different suggestions related to vulnerability fixes for different categories of vulnerabilities, so we suggest that the Rust community could classify vulnerabilities when they are disclosed, or develop automated vulnerability classification tools. We also found that two-thirds of 612 classified vulnerabilities have memory safety or concurrency issues (RQ2), and more efforts are needed to focus on these two kinds of issues to ensure Rust security.

% \noindent\textbf{Unclassified Rust vulnerabilities.}
% 21\% of the reported Rust vulnerabilities (164 out of 776) have not been classified. The lack of classification for vulnerabilities may hurdle the process of vulnerability localization and repair in the Rust ecosystem. 
% %
% Future work could put effort into the development of automated tools to facilitate the classification of vulnerabilities for the Rust ecosystem. 
%Vulnerabilities are not classified. Thus, we need to classify Rust vulnerabilities.

% \noindent\textbf{Rust package categorization.}
% Among the 338 vulnerable packages, 166 packages have not been classified to package functionality categories. Statistics show that these unclassified vulnerable packages are less popular than classified vulnerable packages. And we also found that less popular packages (with less than 100,000 downloads) are prone to suffering from vulnerabilities for more versions, and maintainers of these packages are inactive in fixing vulnerabilities (RQ3). Thus, we recommend contributors in the Rust ecosystem assign tags to promote their packages, which will help the classification of packages and speed up the vulnerability fixing process. What's more, an automatic classification tool for packages should be developed in the future.
\noindent\textbf{\hl{Towards a Safer Rust.}}
 \hl{Given that 77\% of the memory safety and concurrency vulnerabilities are involved in unsafe code (RQ2), software engineers should pay more attention when writing unsafe code to avoid memory safety and concurrency problems. For instance, developers could add Send or Sync bound when implementing Send or Sync trait to avoid data race. In addition, given that tainted input and resource management vulnerabilities reside mostly in safe code (RQ2), developers should pay attention to data validation in safe code when dealing with user input.} 
%Differences exist in the locality of vulnerable code and fixes across various types of Rust vulnerabilities. We make useful suggestions to software engineers and vulnerability researchers for a safer Rust ecosystem. For software engineers, more attention should be paid to write unsafe code related to memory safety problems, because 77\% vulnerabilities of memory safety and concurrency involve unsafe code (RQ2). Specifically, developers should add Send or Sync bound when implementing Send or Sync trait to avoid data race. As discussed in RQ2, \emph{tainted input} and \emph{resource management} vulnerabilities reside mostly in safe code, developers should also check or validate more in safe code when dealing with user input, directory path and etc. 
%For vulnerability researchers, 
%Rust safety mechanisms are effective in preventing memory safety problems and better understand is needed to the potential vulnerable unsafe code. 
%The difference in vulnerability localities suggests that researchers can focus on different code regions when localizing different types of vulnerabilities to save time and effort. 
%We also observe that fixing \emph{exception management} vulnerabilities tend to involve more safe functions compared with other types of vulnerabilities (RQ3). Future work could take into account the types of Rust vulnerabilities for the design of effective Rust program repair tools. 21\% of the reported Rust vulnerabilities (164 out of 776) have not been classified. The lack of classification for vulnerabilities may hurdle the process of vulnerability localization and repair in the Rust ecosystem. Future work could put effort into the development of automated tools to facilitate the classification of vulnerabilities for the Rust ecosystem. By following best practices, we can build a stronger and more secure Rust community.





%(1) Ecosystem 

%     - Ecosystem growth. 
    
%     Javascript: Since its creation in 2009, npm has grown rapidly to now feature over 230, 000 packages (as of January 28th, 2016) the number of packages in Node.js is growing at an accelerated rate~\cite{kikas2017structure,msr2016npm}.
    
%     PyPI: All measures show sustained around 40\% growth rates of new packages over the 13 years (2006 to 2018)~\cite{Bommarito2018PyPI}.
    
%     Java: packages in maven 2004-2017 grows exponentially, 2017-2019 linearly\footnote{\url{https://mvnrepository.com/open-source}}.
    
%     Rust: grows exponentially. Since its creation in 2014, over the last seven years, the ecosystem has rapidly grown and currently hosts over 80,000 packages.
    
%     Rust may suffer from stagnation (mvn) or continue to grow (PyPI).
    
%     - Most popular categories. 
    
%     Javascript: most frequent keywords (i.e., react, api, yeoman-generator, cli and css)~\cite{Lertwittayatrai2017JS}
    
%     PyPi: Software Development is the most common of topics in PyPi packages (37.7\%), Software. Development is over twice as common as the next two most common topics, Internet and Scientific/Engineering. ~\cite{Bommarito2018PyPI}
    
%     Java: Testing Frameworks, Android Packages, Logging Frameworks.\footnote{\url{https://mvnrepository.com/open-source}}
    
%     Rust: Command line utilities, no standard libraries and development tools. 
    
    
    
% (2) Vulnerability distribution. 

%     - All studies found that the number of newly discovered vulnerabilities are growing over time across different ecosystem. What's the possible reasons?
    
%     - The most common vulnerability differs. Memory safety and concurrency issues takes two thirds of vulnerablities in Rust ecosystem, while Cross-Site-Scripting (XSS) is the most common types of vulnerabilities in PyPi and npm ecosystem. Why?
    
%Suggestion on how to automate the fixing of certain types of vulnerabilities. Patch generation, etc. (ICSME 2017)



%\noident\textbf{Comparison with the PyPI ecosystem} [SANER 21 - security vul in python packages]
%\noident\textbf{Comparison with the npm ecosystem} [Usenix security 19 - small world]



==> sections/result_old.tex <==
In this section, we present the results of our research questions that investigate the security risks in the Rust ecosystem. 

%This section presents the results of our research questions from Section 3.1 based on our experiments.
%\subsection{RQ1: Unsafe Rust Usage Analysis.}
%\subsection{RQ1: Characteristics of Rust Ecosystem.}
%\subsection{RQ1: Evolution of the Rust Ecosystem}
% \todo{Xiaoye: I have split the RQ1 section into multiple paragraphs, each paragraph describes a figure; could you please kindly extend each paragraph by detailing more of the findings? may we start with a general idea of the figure, then describe 3 - 5 observations in this figure:-)}
% \zy{@Xiaoye, please refer to MSR 2016 - Section 3, include a paragraph about the total number of packages first;-)}

% The first package in {\tt crates.io} was published on November 11th, 2014. Over the last eight years, the ecosystem has evolved rapidly and currently hosts over 84,105 packages until May 24th, 2022. 
%
%We investigated the evolution of the Rust ecosystem over time and looked for signs of stagnation, i.e., the contribution by the developer community slows down~\cite{msr2016npm}. We also compared the evolution trends across package categories in the Rust ecosystem.
%



% \noindent\textbf{Categorization.}
% 55,895 (66.46\%) packages are not assigned to any categories in {\tt crates.io}. Excluding non-categorized packages, packages are assigned to 1.85 categories on average. The top three categories with the highest numbers are command-line utilities, no std, and development tools, whose package number is over 3000. The category with the lowest numbers is aerospace. It only has 6 crates. The category with the top 3 highest downloads is no-std, development tools, and algorithms, whose number of downloads is over 1,000 million.

%\noindent\textbf{Growth in the number of packages.}
%
% \autoref{fig:numlib} shows the number of packages in the Rust ecosystem over time. As the figure shows, the number of crates created is growing at a rate of 1.5× per year during 2015-2020 on average. When checking the growth rate every year in detail, we discover that the growing rate of the ecosystem slows. The number of crates increases 1.55 times during 2018-2020, but only 1.42 times during 2020-2021. The slowdown may be due to the large base number of libraries, as the absolute number of Rust libraries growing each year is still very large. This may indicate that the Rust ecosystem is still in a phase of rapid growth.


% \autoref{fig:numCreate} shows the number of packages new created every month. As the figure shows, the number new created packages every month is less than 500 in the majority of the month before January 2018, and it is more than 500 after January 2018. Moreover, there are more and more newly created packages every month on the whole. However, there is a continual decrease from August 2020 to November 2020. One explanation for this is developers are concerned about the future of Rust, as some core members are laid off due to the COVID-19. Officially announcing the formation of the Rust Foundation on February 8, 2021, could be a possible reason for the sharp increase in March 2021.

%\noindent\textbf{Number of packages.}
%
%The first package in the Rust ecosystem hosted on {\tt crates.io} was published on November 11, 2014. 
%
%\autoref{fig:numlib} shows the evolution of the number of packages in the Rust ecosystem since its inception. Over the last seven years, the ecosystem has rapidly grown and currently hosts over 80,000 packages. 
%
%The number of packages grows 1.6x per year on average from 2015 to 2020. %
%From 2020 to 2021, the growth in the number of packages slightly slows down, exhibiting a 1.4x growth per year on average.

%Next, we investigated the growth rate of the number of packages in the Rust ecosystem.  \autoref{fig:numCreate} shows the number of packages that are being added to {\tt crates.io} every month. 
%
%\todo{[May 29] We would add footnotes for the news (Rust foundation AND layoff).}\xy{[June 7]Done.}
%The number of packages being created every month has been steadily increasing over time. From late 2014 to early 2018, the increasing number of packages per month is less than 500. Since early 2018, the increasing number of packages per month continues to rise and experiences a peak in March 2021. The peak may be due to the official announcement of the Rust Foundation\footnote{\url{https://foundation.rust-lang.org/news/2021-02-08-hello-world/}} on February 8, 2021, which is an independent non-profit organization to support the set of Rust maintainers that govern and develop the project.
%
%From August 2020 to November 2020, the increasing number of packages per month experiences a sharp decline. %The possible reason for the decline could be the layoff of some core members of Rust in Mozilla%\todo{Specify the organization}
%The possible reason for the decline could be the layoff of active  members in the Rust project at Mozilla (the commercial company originally conceived Rust Project) %\todo{Specify the organization}
%due to the COVID-19 pandemic\footnote{\url{https://blog.rust-lang.org/2020/08/18/laying-the-foundation-for-rusts-future.html}}. 

% \begin{figure}[t]
% \centering
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=6cm]{sections/fig/crates_over_time.pdf}
%         %\caption{Number of Packages Over Time }
%         \caption{Evolution of number of packages.}
%         \label{fig:numlib}
%     \end{minipage}
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=6cm]{sections/fig/crates_every_month.pdf}
%         %\caption{Number of New Packages Created Every Month }
%         \caption{Evolution of number of packages created per month.}
%         \label{fig:numCreate}
%     \end{minipage}

% \end{figure}


%\todo{[May 18] we would further check how the growth differs across categories of crates:-)}\xy{[May 26] Done.}

% We check the growth of the top 6 categories with the highest number of packages, categories with a large number of vulnerabilities (see \autoref{tab:category_percent}), and some other categories with interesting curves. As \autoref{fig:numlib_across_cat} shows, the curve of these top 6 categories seems to resemble the evolution of number of all packages (\autoref{fig:numlib}). The category of memory management and concurrency grows linearly. The category of cryptography has a steep increase between January 2021 and April 2021. This could be also affected by the formation of the Rust Foundation. The category of mathematics and game development starts to grow rapidly from December 2019, which indicates that many other areas begin to choose Rust to program. 

%\todo{[May 29] We may consider top 5 :-)}\xy{[June 7]Done.}
%We further compared the evolution of numbers of packages across categories. As shown in \autoref{fig:numlib_across_cat}, the top 5 categories with the most packages, \emph{command line utilities}, \emph{no std}, \emph{development tools}, \emph{api bindings} and \emph{data structures},  experience a continuous near-exponential growth in the number of packages over time, resembling the growth of the Rust ecosystem. The number of packages in \emph{memory management} and \emph{concurrency} categories grow linearly. The \emph{cryptography} category experiences a steep increase in the number of packages from January 2021 to April 2021. We also observe that the numbers of packages in the \emph{mathematics} and \emph{game development} categories start to grow rapidly since December 2019, indicating practitioners from a variety of areas start to choose Rust for software development.
% We further compared the evolution of the Rust ecosystem in terms of the number of packages across categories. As shown in \autoref{fig:numlib_across_cat}, the top 5 categories with the most packages, \emph{command line utilities}, \emph{no standard library} (a category with packages that are able to function without the Rust standard library), \emph{development tools}, \emph{api bindings} and \emph{data structures}, experience a continuous near-exponential growth in the number of packages over time. The growth in package number of the top 5 categories resembles the growth in package number of the Rust ecosystem. 
% %
% We also observe that the number of packages in \emph{memory management} and \emph{concurrency} categories grow linearly. The \emph{cryptography} category experiences a steep increase in the number of packages from January 2021 to April 2021. 
% %
% In addition, the numbers of packages in the \emph{mathematics} and \emph{game development} categories start to grow rapidly since December 2019, indicating practitioners from a variety of areas start to choose Rust for software development.
%\zy{[May 29] finish polishing in writing for the above results:-)}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{sections/fig/crates_over_time_across_cat.pdf}
%   %\caption{Number of Packages Over Time Across Category}
%   \caption{Evolution of numbers of packages across categories.}
%   \label{fig:numlib_across_cat}
% \end{figure}
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{sections/fig/downloads_over_time_across_cat.pdf}
%   % \caption{Number of Downloaded Packages Over Time across Category (2022-02-24 to 2022-05-23)}
%   \caption{Evolution of package popularity across package categories.} %from October 2022 to May 2022.}
%   \label{fig:numDownload_perCat}
% \end{figure}
% \begin{figure}[t]
% \centering
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=6cm]{sections/fig/crates_over_time_across_cat.pdf}
%         %\caption{Number of Packages Over Time Across Category}
%         \caption{Evolution of numbers of packages across categories.}
%         \label{fig:numlib_across_cat}
%     \end{minipage}
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=6cm]{sections/fig/downloads_over_time_across_cat.pdf}
%         % \caption{Number of Downloaded Packages Over Time across Category (2022-02-24 to 2022-05-23)}
%         \caption{Evolution of package popularity across package categories.} %from October 2022 to May 2022.}
% %        \todo{[Aug 4] Can be make the label larger for each point? and enlarge the font? and please double check the year :-)}
%         \label{fig:numDownload_perCat}
%     \end{minipage}
% \end{figure}


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{sections/fig/categories_crates.pdf}
%   \caption{Number of Libraries In Different Categories}
%   \Description{Number of Libraries In Different Categories}
%   \label{fig:numCategory}
% \end{figure}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{sections/fig/categories_downloads.pdf}
%   \caption{Downloads Of Libraries In Different Categories}
%   \Description{Downloads Of Libraries In Different Categories}
%   \label{fig:numDownload}
% \end{figure}

% There are 52 categories for all libraries\cite{}. For example, the category of algorithms represents Rust implementations of core algorithms such as hashing, sorting, searching, and more. \autoref{fig:numCategory} shows the number of the libraries in 31 categories. Categories with crate numbers under 500 are not shown for a clearer representation. As the figure shows, the top three categories with the highest numbers are command-line utilities, no std, and development tools, whose library number is over 3000. The category with the lowest numbers is aerospace. It only has 6 crates. The category of command-line utilities is a category for applications to run at the command line. The category of no-std categorizes the crates that are able to function without the Rust standard library. The category of development tools includes crates that provide developer-facing features such as testing, debugging, linting, performance profiling, auto-completion, formatting, and more. 

% \autoref{fig:numDownload} shows the number of downloads of libraries in 25 categories. Categories with download number under 100,000,000 are not represented in the \autoref{fig:numDownload}. As shown in Figure~\ref{fig:numDownload}, the category with the highest downloads is no-std, whose number of downloads is over 3,344 million. Compared to the two treemaps, we could find that some categories (e.g., command-line-utilities, web-programming) have a great number of crates but low downloads.


%\noindent\textbf{Package popularity.}
%\zy{[May 29] Evolution of downloads over time; will we use the complete data to update the results? Daily downloads OR monthly downloads?} \xy{[June 7] Update with complete data. Monthly downloads.}

%We investigate the downloads of all Rust packages on a monthly basis from November 2014 to May 2022. As \autoref{fig:downloadEvolution} shows, the number of package downloads grows exponentially over time. The growth rate of package downloads has been increasing dramatically since April 2019, which is far greater than the growth rate of package numbers, indicating an active and growing Rust ecosystem.
%
%\todo{We may answer: What are the most popular category, or even most popular package? this help us dig deep for RQ2.}\xy{[May 27] Done.}
%The top 3 most popular packages are {\tt time}, {\tt libc} and {\tt crossbeam-utils}, each of which has over 35 million downloads in total. 
%\todo{[Jun 20] @Xiaoye, so the downloads in during the last three months?}
%In addition, we observe that the {\tt hyper}, {\tt smallvec}, {\tt openssl-sys} and {\tt rusqlite} packages have gained popularity recently, with 20,825,352, 10,650,620, 9,994,576 and 860,053 downloads from March 2022 to May 2022. 
%

% \begin{figure}[t]
% \centering
% %    \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=0.5\textwidth]{sections/fig/crates_over_time_across_cat.pdf}
%         %\caption{Number of Packages Over Time Across Category}
%         \caption{Evolution of numbers of packages across package categories.}
%         \label{fig:numlib_across_cat}
% %    \end{minipage}


% \end{figure}

% \begin{figure}[t]
% \centering
%         \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=6cm]{sections/fig/downloads_evolution.pdf}
%         %\caption{Number of Downloaded Packages Every Day (2022-02-24 to 2022-05-23)}
%         \caption{Evolution of package popularity.}% (2014-10 to 2022-05).}
%         \label{fig:downloadEvolution}
%     \end{minipage}
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=6cm]{sections/fig/downloads_over_time_across_cat.pdf}
%         % \caption{Number of Downloaded Packages Over Time across Category (2022-02-24 to 2022-05-23)}
%         \caption{Evolution of package popularity across package categories.} %from October 2022 to May 2022.}
% %        \todo{[Aug 4] Can be make the label larger for each point? and enlarge the font? and please double check the year :-)}
%         \label{fig:numDownload_perCat}
%      \end{minipage}
%     % \zy{[Aug 13] below figure is not referenced in the paper :-)}
%     % \begin{minipage}{0.48\textwidth}
%     %     \centering
%     %     \includegraphics[width=6cm]{sections/fig/downloads_every_month.pdf}
%     %     \caption{Evolution of package downloads per month.}
%     %     \label{fig:numDownload_perMon}
%     % \end{minipage}
% \end{figure}

%\todo{[May 18] we would check how the growth differs across categories of crates:-)}\xy{[May 27] Done.}
%\zy{[May 29] Evolution of downloads across categories of packages. (Let's organize the paragraph as ``number of packages''.) (1) top 5 categories with the most downloads (2) exponential growth (3) linear growth (4) other interesting growth:-)}
%\xy{[June 7] Done. No linear growth.}

%We then investigated the evolution of package downloads across categories. As shown in \autoref{fig:numDownload_perCat}, %\yun{check again, the top 5 categories with the most packages are: command-line utilities, no std, development tools, API bindings, and data structures?}\xy{Yes.} 
%the top 5 categories with the most packages, \emph{no standard library}, \emph{development tools}, \emph{algorithms}, \emph{data structures} and \emph{asynchronous}, experience a continuous near-exponential growth in downloads over time, resembling the growth of package download in the Rust ecosystem. %The \emph{caching} category experiences a steep increase in downloads from December 2021 to February 2022. %We observe that categories with a large number of vulnerabilities (see \autoref{tab:category_percent}) are widely downloaded.


% \zy{[May 29] build connection between NUMBER of PACKAGES and Popularity -- (compare the ranks of categories across these two parts :-))}\xy{Done.}
% Comparing \autoref{fig:numlib_across_cat} and \autoref{fig:numDownload_perCat}, we find that \emph{command line utilities} has large number of crates and grows rapidly, but it is rarely downloaded over the time. \emph{API bindings} ranks top 5 in the number of packages but it grows near-linearly in downloads. Besides, \emph{memory management} and \emph{concurrency} categories grow linearly in the number of packages but their downloads grow rapidly in an exponential rate.
%We further compared the ranks of package categories in terms of package numbers and popularity. We observe that the \emph{command line utilities} category has a large number of packages and grows rapidly in terms of package number, but attracts limited downloads over time. The \emph{API bindings} category ranks in the top 5 in terms of package number, but ranks out of the top 5 in terms of package downloads, experiencing a near-linearly growth in downloads. Besides, the \emph{memory management} and \emph{concurrency} categories grow linearly in terms of package numbers but grow exponentially in terms of downloads.

%\vspace{-0.2cm}
% \begin{tcolorbox}[width=\linewidth,
%                   boxrule=0.5pt,
%                   arc=0mm,
%                   left=0pt,
%                   right=0pt,
%                   top=2pt,
%                   colback=yellow!30]

% \textbf{Summary for RQ1:} %\todo{[Jun 22] @Xiaoye, please summarize each RQ with 4-6 sentences, each sentence summarizes one paragraph :-)}
% The Rust ecosystem actively grows explosively in the number and popularity of packages. 
% %
% %An increasing number of areas start to choose Rust for software development. 
% %
% The increasing number of Rust packages per month experiences a decline from August 2020 to November 2020 due to the COVID-19 pandemic, and continues to rise and reach a peak in March 2021.
% %
% The number of packages in less popular categories increases rapidly since December 2019, indicating that practitioners from a variety of areas start to choose Rust for software development.
% %
% The growth in the number and popularity of packages varies across different package categories. The \emph{data structures}, \emph{no standard library} and \emph{development tools} packages rank the top 3 in terms of both number and popularity of packages.

% \end{tcolorbox}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{sections/fig/downloads_over_time_across_cat.pdf}
%   % \caption{Number of Downloaded Packages Over Time across Category (2022-02-24 to 2022-05-23)}
%   \caption{Evolution of package popularity across package categories.} %from October 2022 to May 2022.}
%   \label{fig:numDownload_perCat}
% \end{figure}


% \todo{We may answer: What are the most popular category, or even most popular package? this help us dig deep for RQ2.}\xy{[May 27] Done.}
% % The package of {\tt time}, {\tt libc} and {\tt crossbeam-utils} are most downloaded packages, whose downloads are above 35,000,000. 
% The top 3 most popular packages are {\tt time}, {\tt libc} and {\tt crossbeam-utils}  with over 35 million downloads.
% %
% \zy{[May 29] What do you mean by "recently" exactly?}\xy{[June 7] Update. }
% The packages of {\tt hyper} (20,825,352), {\tt smallvec} (10,650,620), {\tt openssl-sys} (9,994,576) and {\tt rusqlite} (860,053) are also widely downloaded in recent three month (from March 2022 to May 2022). 


%\subsection{RQ2: Library Vulnerability Analysis}
\subsection{RQ1: Vulnerabilities in the Rust Ecosystem}
We investigated the characteristics of disclosed vulnerabilities in the Rust ecosystem, including the vulnerability types, life spans, and the evolution of the number of vulnerabilities.
%
%\todo{[Jun 20] We may consider adding a new RQ - for vulnerable packages. (Risks in the Rust ecosystem)}
%In addition, we characterized the vulnerable packages in terms of types and numbers of disclosed vulnerabilities, affected versions, and package categories.

% \zy{methodology - dataset stats.}
% We crawled 776 vulnerabilities on May, 21st, 2022. 

%\noindent\textbf{Types of vulnerabilities.}
%\zy{[May 30] we may clarify xxx vulnerabilities do not have categories in Methodology.}
%\zy{OLD.}
%We used primary clusters of SFP to categorize the vulnerabilities. 167 vulnerabilities are not categorized by CWE or categories. Excluding non-categorized vulnerabilities, we observed that the average number of categories per vulnerability was 1.23 (median = 1, maximum = 3). 
%\todo{NEW.}
%We collected a total of 776 unique vulnerabilities in the Rust ecosystem, of which 164 have not been categorized. Among the 612 vulnerabilities, we identified an average of 1.2 vulnerability types for each vulnerability (min: 1, max: 3, median: 1, std: 0.44). The overall distribution of vulnerabilities across 612 vulnerability types is presented in \autoref{tab:cve_tpe}.
\begin{table}[t]
  \caption{Distribution of vulnerabilities across vulnerability types.}
%  \caption{Vulnerability types.}
  \label{tab:cve_type}
  \small
  \begin{tabular}{lllp{3.3cm}p{3cm}}
    \toprule
%    Vulnerability types & Vulnerability & Percentage\\
    \textbf{Vulnerability Type} & \textbf{Count} & \textbf{Percentage} & \textbf{Duration between Introduction and Disclosure (Days in Median)} & \textbf{Duration between Disclosure and Fixing (Days in Median)}\\
    \midrule
    Memory Management       & 144       & 24.24\% & 989  &213\\
    Memory Access           & 141       & 23.74\% & 1,053 &219\\
    Synchronization         & 74        & 12.46\% & 1,004 &217\\
    Tainted Input           & 46        & 7.74\%  & 1,070 &201\\
    Resource Management     & 40        & 6.73\%  & 1,341 &316\\
    Exception Management    & 38        & 6.40\%  & 1,278 &225\\
    Cryptography            & 26        & 4.38\%  & 1,075 &459\\
    Other                   & 26        & 4.38\%  & 1,392 &354\\
    Risky Values            & 21        & 3.54\%  & 1,384 &52\\
    Path Resolution         & 14        & 2.37\%  & 858  &37\\
    Information Leak        & 9         & 1.52\%  & 277  &364\\
    Privilege               & 4         & 0.67\%  & 277  &36\\
    Predictability          & 3         & 0.51\%  & 277  &148\\
    Authentication          & 3         & 0.51\%  & 1,406 &1,624\\
    API                     & 2         & 0.34\%  & 1,264 &658\\
    Access Control          & 2         & 0.34\%  & 304  &82\\
    Failure to Release Memory & 1       & 0.17\%  & 918  &192\\
    \bottomrule
  \end{tabular}
\end{table}

\noindent\textbf{Types of vulnerabilities.} We collected a total of 433 unique vulnerabilities in the Rust ecosystem, out of which 73 have not been categorized, \hl{leaving 360 vulnerabilities that are categorized with a median of 1 vulnerability type (min: 1, max: 4, mean: 1.65, std: 0.76).} \autoref{tab:cve_type} presents the overall distribution of vulnerabilities across 17 vulnerability types. Memory safety and concurrency issues account for two-thirds of the 433 vulnerabilities.

%\zy{OLD. We would thoroughly discuss top vulnerability types a little bit:-)}
%\autoref{tab:cve_tpe} presents distribution of vulnerabilities over SFP. Excluding those not classified vulnerabilities, We can observe that the top three vulnerability types are Memory Access (23.08\%), Memory Management (21.62\%), and Synchronization (18.83\%). Access Control (0.27\%) and API (0.27\%) are rare in Rust-related vulnerabilities. Memory safety issues and concurrency problems account for two-thirds of all the categorized vulnerabilities, suggesting that Rust still cannot avoid memory issues in practice. 

%\todo{NEW.}
%Most of the vulnerabilities are labeled as \emph{memory access} (23.08\%) and \emph{memory management} (21.62\%) problems. %\todo{[Jun 1] We would explain the difference between memory access and memory management a little bit; one sentence first; two CVE examples further:-)}\xy{[June 9] Done.}
%\emph{memory access} is a category of vulnerabilities with memory access problems, commonly in buffer or pointer access. \emph{buffer overflow}, \emph{use after free} and \emph{null pointer dereference} are belong to \emph{memory access} category. \emph{memory management} is a category with memory allocation or free problem. \emph{double free} is belong to \emph{memory management}. For example, RUSTSEC-2021-0128 is a \emph{memory access} vulnerability in rusqlite package. The lifetime bound on several closure-accepting rusqlite functions is so relaxed that it could allow Rust code to access objects on the stack after they have been dropped, which causes \emph{use after free}. RUSTSEC-2021-0033 is an example for \emph{memory management}. {\tt push\_cloned} function in {\tt stack\_dst} package can drop uninitialized memory or double free on panic. Memory safety issues and concurrency problems account for two-thirds of all the categorized vulnerabilities, suggesting that Rust still cannot avoid memory issues in practice. 
Memory safety issues involve \emph{memory access} (23.74\%) and \emph{memory management} (24.24\%) vulnerability types, accounting for almost half of the categorized vulnerabilities. 
%
The \emph{memory access} vulnerabilities usually arise from buffer or pointer access problems, e.g., \textit{buffer overflow}, \textit{use after free}, and \textit{null pointer deference}. We take the RUSTSEC-2021-0128 in the {\tt rusqlite} package as an example of \emph{memory access} vulnerability. In the vulnerable code of the {\tt rusqlite} package affected by RUSTSEC-2021-0128, the lifetime bounds on several closure-accepting functions are so loose that allow the access to dropped objects on the stack thus cause \textit{use after free} error.
% 
The \emph{memory management} vulnerabilities are due to problems in memory allocation or deallocation, e.g., \textit{double free}. RUSTSEC-2021-0033 in the {\tt stack\_dst} package is an example of \emph{memory management} vulnerabilities. Specifically, the {\tt push\_cloned} function in the vulnerable code of {\tt stack\_dst} package deallocates uninitialized memory thus cause \textit{double free} error.
%
Concurrency issues involve \emph{synchronization} vulnerabilities, which rank the third in the frequency of occurrence across different types of vulnerabilities (12.46\%). 
The \emph{Synchronization} vulnerabilities occur when multiple processes or threads share resources, including race condition and misuse of locks. For instance, the unsafe {\tt Send} trait implementation in the {\tt atom} package involved in RUSTSEC-2020-0044 causes data race error.
% \emph{Synchronization} vulnerabilities rank the third in the frequency of occurrence (12.46\%). The \emph{synchronization} type of vulnerabilities represent the problems with sharing resources, including  \emph{race condition} and \emph{missing lock}. RUSTSEC-2020-0044 is  an example of \emph{synchronization} vulnerabilities in the {\tt atom} package. The unsafe \emph{Send} trait implementation in {\tt atom} causes data race.

\noindent\textbf{Vulnerability life spans.}
We observed that vulnerabilities exist in code repositories for extensive duration. Specifically, it takes an average of 1,155 days (3.2 years) for a vulnerability to be disclosed after the vulnerability was introduced in a Rust package (median: 1,125, min: 25, max: 2,726, std: 684.1). Looking at per-vulnerability medians, we see that 50\% of the vulnerabilities had disclosure duration exceeding 1,125 days (3.1 years). 
% max disclosure duration
The vulnerability with the longest disclosure duration (2,726 days) was RUSTSEC-2022-0022 in the \emph{hyper} package, introduced in May 2018 and disclosed in May 2022. 
% (2,642 days) was RUSTSEC-2022-0013 in the \emph{regex} package, introduced in December 2014 and disclosed in March 2022. 
% min disclosure duration
%【Min -- 小叶，能否看下这些时间较短的vul的introduce分布 -- 如果时间呈现靠近近期的倾向，咱们可以多说一些，可能是由于Rust ecosystem的security awareness增强了!】
In addition, 1.4\% of the vulnerabilities had a disclosure duration lower bound of less than 30 days. The average time of vulnerability introduction for those with a disclosure duration of less than 300 days is October 2020, while the average time of introduction for all vulnerabilities is January 2018. This may indicate an increase in security awareness within the Rust ecosystem.


Meanwhile, we observed that vulnerabilities remain unpatched when disclosed for extensive duration. 156 out of 433 vulnerabilities remained unpatched in May 2022. Specifically, it takes an average of 368 days (1 year) for a vulnerability to be fixed after its disclosure in the Rust ecosystem (median: 212, min: 2, max: 1,934, std: 410.8). Looking at per-vulnerability medians, we see that 50\% of the vulnerabilities remained unaddressed 212 days after disclosure, leaving a wide window open for attacker exploitation.
%【Max - 1,934 - 这个已经被fix了吗？没有的话，可以聊一下这个CVE哈】此处所有的统计都是对fixed vulnerability做的
Approximately xx\% of the vulnerabilities remained unpatched over 180 days after their disclosure.

\hl{We calculated the time between the vulnerabilities introduced and disclosed.} As shown in \autoref{fig:introVulnerability}, \hl{the number of introduced vulnerabilities grows linearly from November 2014 to January 2020 ($R^2=0.9918$), and becomes stabilized after March 2020. It takes an average of 1,155 days, which is around 3.2 years, for a vulnerability to be disclosed after its introduction in a Rust package (median: 1,125, min: 25, max: 2726, std: 684.1). Meanwhile, it takes an average of 368 days for a vulnerability to be fixed after its disclosure  (median: 212, min: 2, max: 1,934, std: 410.8). }
%
\hl{Our findings is consistent with other ecosystems--vulnerabilities in npm packages and PyPI take at least 3 years to be discovered and made public}~\cite{decan2018impact, alfadel2021empirical}.
%
\hl{We also studied the disclosure and fix duration across vulnerability types, } as shown in \autoref{tab:cve_type}. We observe that vulnerability disclosure and fix duration vary widely based on the vulnerability types. For the top 5 vulnerability types, \emph{resource management} has significantly longer duration both in disclosure and fix, suggesting that the vulnerabilities in \emph{resource management} are more challenging to disclose and fix.

\noindent\textbf{Vulnerability evolution.}
%
% \autoref{fig:numVulnerability} shows the number of disclosed vulnerabilities in the lifetime of the ecosystem. \autoref{fig:numVulnerability} has a steep increase in the last two years. To explore this relationship further we plot in \autoref{fig: Vulnerabilityrate} the evolution of the number of vulnerabilities disclosed per 1,000 crates and we observe that it grows from one in 2017 to almost five in 2022. This is a sign of a healthy security community that reports vulnerabilities at a very good pace, keeping up with the growth of the ecosystem.
% We investigated the evolution of the number of disclosed vulnerabilities in the Rust ecosystem.
% \autoref{fig:numVulnerability} shows the number of disclosed vulnerabilities in the lifetime of the ecosystem. 
% \todo{[Jun 1] We may say more about the trend of this curve :-) 1) grows slowly and reaches 100 in month year; 2) first rapid growth in month year, try to explain why; 3) second rapid growth in month year, try to explain why.}\xy{[Jun 8] Done.}
% The number of exploited vulnerabilities in the ecosystem grows slowly from November 2014 to November 2020. Then it experiences first rapid growth from November 2020 to March 2021. One explanation for the first rapid growth is that a large-scale campaign is carried out during this period: there are 129 memory safety and soundness vulnerabilities disclosed in Rustsec as part of the research efforts of Yechan Bae\cite{Rudra}. The second rapid growth in August 2021 is nearly vertical, increasing from 333 to 633. A vulnerability pattern of an unrestricted {\tt Send} or {\tt Sync} on generic types discovered by Rudra team\cite{Rudra} disclosed in GitHub Advisory contributes to about a one-third increase.
%
We present the evolution of the number of vulnerabilities discolsed over time in the Rust ecosystem in \autoref{fig:numVulnerability}. We observe that the number of vulnerabilities disclosed grows slowly from November 2014 to November 2020, and experiences two rapid growth phases. The first rapid growth starts from November 2020 and ends in March 2021, while the second occurs in July 2021. The first rapid growth may attribute to a large-scale campaign during that period of time, in which RustSec has published 129 memory safety vulnerabilities as part of the research efforts made by Bae et al. ~\cite{Rudra}. During the second rapid growth, the number of disclosed vulnerabilities increased from 197 to 330 due to unrestricted {\tt Send} or {\tt Sync} on generic types, which is also discussed in prior work~\cite{Rudra}. 
%
The evolution in the numbers of vulnerabilities vary widely across vulnerabilities types as shown in \autoref{fig:numVulAcrossType}. The \emph{memory access}, \emph{memory management} and \emph{synchronization} vulnerabilities grow fastest over time, with a growth pattern that resembles the evolution of vulnerabilities disclosed in the Rust ecosystem as shown in \autoref{fig:numVulnerability}.
%
We also present the evolution of the number of vulnerabilities introduced into Rust code repositories over time in \autoref{fig:introVulnerability}, which demonstrates a linear growth rate from November 2014 to January 2022 ($R^2$ = 0.9918) and becomes stabilized after March 2020. The numbers of vulnerabilities disclosed and introduced demonstrate different growth rates over time, which may be due to the increase of individuals and organizations participated in Rust vulnerability discovery as Rust becomes increasingly popular in systems software development. Another possible reason could be the development and application of vulnerability detection tools in the Rust ecosystem, which facilitate the discovery of vulnerabilities~\cite{Rudra,li2021mirchecker}.

Next, we investigated whether package growth in the Rust ecosystem contributes to the increase of disclosed vulnerabilities. As shown in \autoref{fig:Vulnerabilityrate}, the normalized number of vulnerabilities disclosed per 1,000 packages grows from one in 2017 to five in 2022, indicating an increase of package-wise security risks in the Rust ecosystem. Meanwhile, the normalized number of vulnerabilities disclosed per 100,000 lines of code in vulnerable packages reaches the peak (2.1) in August 2020 after three climbing stages, and have experienced a sharp decrease to 0.5 since then, as shown in \autoref{fig:VulnerabilityLoc}, suggesting a decreasing tendency in security risks per lines of code in the Rust ecosystem.

Finally, we investigated how vulnerabilities with different types evolve over time with respect to package category as shown in \autoref{fig:numVulAcrossCategory}. We make several observations:
\begin{itemize}
\item \emph{Memory management} vulnerabilities are disclosed across package categories, but with different frequencies of occurrence and growth rates.
\item \emph{Command line utilities} packages have no vulnerability disclosed until April 2021, and have 12 vulnerabilities disclosed in total until April 2022, indicating relatively low security risk over time (\autoref{subfig:cmd}). 
\item \emph{No standard library} and \emph{data structures} packages both have more than 60 vulnerabilities disclosed in total until April 2022, among which \emph{memory management} vulnerabilities account for a majority (\todo{xx}\% in \emph{no standard library} and \todo{xx}\% in \emph{data structures}) (\autoref{subfig:no-std} and \autoref{subfig:ds}). The numbers of disclosed vulnerabilities are greater than any other package categories, indicating relatively high security risk over time. 
\end{itemize}
%\hl{To get the better understand of the security risks in the ecosystem, we normalized the number of disclosed vulnerabilities to lines of code (LOC) of vulnerable packages,} as shown in \autoref{fig:VulnerabilityLoc}. \hl{Note that we excluded the vulnerabilities whose package has no recorded LOC in the dataset. The data before February 2018 is imprecise here, because it only contains 1 vulnerability. From November 2019 to June 2021, we see that the security risks steadily grow. Its trend is the same as the number of vulnerabilities evolution. After July 2021, the security risks decline. One possible reason could be the second rapid growth of the vulnerabilities examined more vulnerable packages, which leads to LOC of the vulnerable packages grow rapidly and security risks decline. In total, the security risks of the ecosystem is at a low level with 1 vulnerability per 100,000 lines.}
Furthermore, we investigated whether the growth in package numbers leads to an increase in the number of disclosed vulnerabilities. As shown in \autoref{fig:Vulnerabilityrate},  the vulnerabilities disclosed per 1,000 packages grows from one in 2017 to five in 2022. 
As shown in \autoref{fig:VulnerabilityLoc}, \hl{the normalized number of disclosed vulnerabilities fluctuates around 1 per 100,000 lines of code. Notably, the normalized number of vulnerabilities in vulnerable packages has decreased since October 2020, despite the rapid growth of disclosed vulnerabilities in the Rust ecosystem. }

\begin{figure}[t]
\centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=6.5cm]{sections/fig/vulnerabilities_over_time.pdf}
        %\caption{Number of Vulnerabilities Published over Time}
        \caption{Evolution of number of disclosed vulnerabilities.}
        \label{fig:numVulnerability}
    \end{minipage}
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{sections/fig/vul_overtime_across_type.pdf}
        \caption{Evolution of numbers of disclosed vulnerabilities across vulnerability types.}
        \label{fig:numVulAcrossType}
    \end{minipage}
    
    
\end{figure}

\begin{figure}[t]
\centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=6.5cm]{sections/fig/vulnerabilities_introduced_over_time.pdf}
        \caption{Evolution of number of introduced vulnerabilities.}
        %\todo{[Jun 1] the x axis would be consistent with that of \autoref{fig:numVulnerability}}
        \label{fig:introVulnerability}
    \end{minipage}
    % \begin{minipage}{0.48\textwidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{sections/fig/vul_overtime_across_package.pdf}
    %     \caption{Evolution of numbers of disclosed vulnerabilities across package categories.}
    %     \label{fig:numVulAcrossCategory}
    % \end{minipage}
\end{figure}
%
%The number of vulnerabilities in the Rust ecosystem experiences a steep increase during the last one and half years, increasing from \todo{xxx} to \todo{xxx}. 
%
%\zy{below from the old version; is it the reason for some interesting points in the evolution?}
% We observe that almost 30\% of the advisories come from a large-scale campaign and not a broader community effort: there are 129 memory safety and soundness vulnerabilities disclosed as part of the research efforts of Yechan Bae\cite{Rudra}. Nevertheless, this shows the feasibility of large-scale vulnerability detection and reporting on Rust.
% \todo{[Jun 1] @Xiaoye, this analysis may help to understand if the increase in vul number is because of the increase in package number.}
% We explored the reason for the sharp increase in the number of vulnerabilities since December 2021. We check if the growth of the Rust ecosystem leads to an increase in the number of vulnerabilities. As shown in \autoref{fig: Vulnerabilityrate}, the number of vulnerabilities disclosed per 1,000 crates grows from one in 2017 to almost five in 2022. This is a sign of a healthy security community that reports vulnerabilities at a very good pace, keeping up with the growth of the ecosystem.
%

%\hl{Moreover, we studied the evolution of the number of introduced vulnerabilities based on their published date of the earliest affected version. Note that we take the published date of the earliest affected version as the introduced date rather than blame the vulnerable code to find the exact written date of the vulnerable code. As represented in \autoref{fig:introVulnerability}, the number of introduced vulnerabilities grows linearly from November, 2014 to January, 2020 ($R^2=0.9861$). The curve goes flat after March 2020. One possible reason is that potential vulnerabilities have not been disclosed or disclosed so far and we cannot get the version to blame for the undiscovered vulnerabilities. We calculated the time between the vulnerabilities introduced and disclosed. It takes 1159 days (around 3.2 years) on average (median: 1086, min: 2, max: 2726, std: 688.7） for an introduced vulnerabilities to be disclosed. The time between the vulnerabilities disclosed and fixed version release is 360 days on average (median: 216, min: 1, max: 1934, std: 377.1).}


As shown in \autoref{fig:numVulnerability} and \autoref{fig:introVulnerability}, \hl{the number of introduced vulnerabilities grows linearly from 2017 to 2022, but the number of disclosed vulnerabilities experiences rapid growth. One possible reason may be the increased involvement of individuals and organizations in vulnerability discovery as Rust becomes increasingly popular in software development. Another possible reason may be the development and application of vulnerability detection tools in the Rust ecosystem facilitate the discovery of vulnerabilities}~\cite{Rudra,li2021mirchecker}.
%As shown in \autoref{fig:Vulnerabilityrate}, the number of vulnerabilities disclosed per 1,000 packages grows from one in 2017 to almost five in 2022. Multiple factors may cause the increasing. One possible factor may be that developers simply include more bugs when writing the packages. Another factor may be more researchers or organizations are involved in discovery of vulnerabilities and automatic vulnerability-detection tools like fuzzing get more popular and applied. From \autoref{fig:introVulnerability}, \hl{we see that vulnerabilities introduced grows linearly, but the vulnerabilities disclosed per 1,000 packages grows to 5, which means more efforts are paid to find out vulnerabilities in the ecosystem.} %This is a sign of a healthy security community that reports vulnerabilities at a good pace, keeping up with the growth of the ecosystem~\cite{zimmermann2019small}.
% \zy{seems different compared to the evolution of the number of packages:-)}
% The curve seems to resemble the evolution of the number of packages presented in \autoref{fig:numlib}.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{sections/fig/vulnerabilities_over_time.pdf}
%   %\caption{Number of Vulnerabilities Published over Time}
%   \caption{Evolution of number of disclosed vulnerabilities.}
%   \label{fig:numVulnerability}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{sections/fig/vulnerabilities_crates_over_time.pdf}
%   \caption{Rate of published vulnerabilities per 1,000 packages.}
%   \todo{[Jun 1] the x axis would be consistent with that of \autoref{fig:numVulnerability}}
%   \label{fig:Vulnerabilityrate}
% \end{figure}




\begin{figure}[t]
\centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=7cm]{sections/fig/vulnerabilities_crates_over_time.pdf}
        \caption{Disclosed vulnerabilities per 1,000 packages.}
        %\todo{[Jun 1] the x axis would be consistent with that of \autoref{fig:numVulnerability}}
        \label{fig:Vulnerabilityrate}
    \end{minipage}
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=6.5cm]{sections/fig/vulnerabilities_norm_loc.pdf}
        % \caption{disclosed vulnerabilities normalized by vulnerable packages' lines of code.}
        \caption{Disclosed vulnerabilities per vulnerable packages' lines of code.}
        \label{fig:VulnerabilityLoc}
    \end{minipage}
    
\end{figure}


% \begin{figure}[t]
% \centering
%     \centering
%     \includegraphics[width=\linewidth]{sections/fig/vul_overtime_across_package.pdf}
%     \caption{Evolution of numbers of disclosed vulnerabilities across package categories.}
%     \label{fig:numVulAcrossCategory}
% \end{figure}

\begin{figure}[t]
    \centering
    \captionsetup[subfigure]{font=tiny}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\linewidth]{sections/fig/vul_package_No standard library.pdf}
        \caption{No standard library}
        \label{subfig:no-std}
    \end{subfigure}
\hfil
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\linewidth]{sections/fig/vul_package_Development tools.pdf}
        \caption{Development tools}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\linewidth]{sections/fig/vul_package_Command line utilities.pdf}
        \caption{Command line utilities}
        \label{subfig:cmd}
    \end{subfigure}
\hfil
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\linewidth]{sections/fig/vul_package_Data structures.pdf}
        \caption{Data structures}
        \label{subfig:ds}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\linewidth]{sections/fig/vul_package_Memory management.pdf}
        \caption{Memory management}
    \end{subfigure}
\hfil
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\linewidth]{sections/fig/vul_package_Web programming.pdf}
        \caption{Web programming}
    \end{subfigure}

    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\linewidth]{sections/fig/vul_package_Asynchronous.pdf}
        \caption{Asynchronous}
    \end{subfigure}
\hfil
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\linewidth]{sections/fig/vul_package_Cryptography.pdf}
        \caption{Cryptography}
    \end{subfigure}
    \caption{Evolution of numbers of disclosed vulnerabilities across package categories.}
    \label{fig:numVulAcrossCategory}
\end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.6\linewidth]{sections/fig/vul_overtime_across_type.pdf}
%   \caption{Evolution of numbers of disclosed vulnerabilities across vulnerability types.}
%   \label{fig:numVulAcrossType}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.6\linewidth]{sections/fig/vul_overtime_across_package.pdf}
%   \caption{Evolution of numbers of disclosed vulnerabilities across package categories.}
%   \label{fig:numVulAcrossCategory}
% \end{figure}

% \todo{[Jul 1] We would compare evolution across vulnerability types.}
% \xy{[Jun 8] Done.}
% We further compared the evolution of numbers of vulnerabilities across various types of vulnerabilities. As shown in \autoref{fig:numVulAcrossType}, the top 5 types with the most vulnerabilities, \emph{memory access}, \emph{memory management}, \emph{synchronization} experience two rapid growth over time, resembling the growth of the Rust ecosystem. \emph{Resource management}, \emph{tainted input} and \emph{cryptography} only experience the latter rapid growth in the Rust ecosystem, which is consistent with the first rapid growth caused by memory safety issues. \emph{Exception management} starts to grow linearly from August 2021, suggesting that another vulnerability type is discovered in the Rust ecosystem. 
We further compared the evolution of the numbers of vulnerabilities across various vulnerability types. As shown in \autoref{fig:numVulAcrossType}, the top 3 vulnerability types with the fastest growth rate in the Rust ecosystem, \emph{memory access}, \emph{memory management}, \emph{synchronization}, experience two rapid growth phases in the numbers of vulnerabilities, resembling the evolution of vulnerabilities in the Rust ecosystem (\autoref{fig:numVulnerability}).
% finish above
%\todo{[Jun 21] @Xiaoye, what do you mean by ``latter'' and ``consistent with the first rapid growth''?}
The vulnerabilities of \emph{resource management}, \emph{tainted input} and \emph{cryptography} types experience a  rapid growth from July 2021 to August 2021. % In addition, the \emph{exception management} types of vulnerabilities emerge after August 2021.
%\todo{[Jun 27] from July, 2021 to August, 2021}. %, which is consistent with the first rapid growth caused by memory safety issues. 
% finish below

 % and its number grows near linearly over time. %, suggesting that another vulnerability type is discovered in Rust ecosystem. 
\hl{We also investigated how vulnerabilities with different types evolve grouped by package category. In general, the evolution of vulnerabilities grouped by various package categories, as depicted in}~\autoref{fig:numVulAcrossCategory}, \hl{exhibits a similar trend to the overall evolution of vulnerabilities presented in}~\autoref{fig:numVulnerability}. \hl{ The packages categories of \emph{command line utilities} has only 12 vulnerabilities in April 2022 and did not have a disclosed vulnerabilities until 2021, which indicates the package category is at low security risks. The vulnerabilities in the categories of \emph{data structures} and \emph{no standard library} grow to more than 50. }%\hl{The reason why different categories of vulnerabilities exhibit similarity in their evolution could be attributed to the broad scope of vulnerability hunting rather than targeting specific categories.} 
\hl{In terms of distribution of vulnerability types, we observed that common types of vulnerabilities have been disclosed across package categories, e.g., the \emph{memory management} vulnerabilities. }
% Specific types of vulnerabilities tend to relate with particular package categories. For instance, the \emph{cryptography} vulnerabilities  dominate the vulnerabilities that are disclosed in the packages of cryptography category; The \emph{synchronization} vulnerabilities account for a large portion of vulnerabilities in No standard library, Memory management and Asynchronous categories of packages

%\hl{We also investigated the evolution of vulnerabilities with different types grouped by package categories.} As shown in \autoref{fig:numVulAcrossCategory}, \hl{the evolution across different package categories behaves similarly as the total evolution in }~\autoref{fig:numVulnerability}. \hl{One possible reason for the similarity across different categories is that the vulnerability hunting dose not focus on a specific category and the vulnerabilities disclosed so far are common types.} The \emph{cryptography} type mostly exist in cryptography package categories. The \emph{memory access} shares in all package categories. The categories of No standard library, Memory management and Asynchronous have large portion of \emph{synchronization} types and grow rapidly after August 2021. 

\vspace{-0.2cm}
\begin{tcolorbox}[width=\linewidth,
                  boxrule=0.5pt,
                  arc=0mm,
                  left=0pt,
                  right=0pt,
                  top=2pt,
                  colback=yellow!30]

\textbf{Summary for RQ1:} 
%Two-thirds of 612 vulnerabilities have memory safety or concurrency issues. The evolution of vulnerabilities experiences two rapid growth, both of which are caused by a large-scale vulnerability campaign. The number of vulnerabilities disclosed per 1,000 packages grows from one in 2017 to almost five in 2022, suggesting a healthy security community., suggesting a healthy security community.

The \emph{memory access}, \emph{memory management} and \emph{synchronization} vulnerabilities account for 60\% of the disclosed vulnerabilities in the Rust ecosystem, exhibiting the fastest growth rates. The number of disclosed vulnerabilities experiences two rapid growth periods, in November 2020 and August 2021, both of which are caused by a large-scale vulnerability campaign. The number of introduced vulnerabilities grows linearly and it takes around 3 years for an introduced vulnerabilities to be published. 
\end{tcolorbox}

%
\subsection{RQ2: Vulnerable Packages in the Rust Ecosystem}\label{sec:result_RQ2}
%\noindent\textbf{Vulnerable Rust packages.}
% We obtained a total of 338 vulnerable packages, accounting for 0.40\% of packages in the Rust ecosystem. The 338 vulnerable packages have an average of 2.3 disclosed vulnerabilities (min: 1, max: 18, median: 2, std: 1.83), affecting 79.92\% version of each package on average (min: 1.39\%, max: 100\%, median: 87.75\%, std: 0.235) and 19.6 versions of each package on average in absolute (min: 1, max: 210, median: 12, std: 24.65). Note that there are 120 vulnerable packages that remained unpatched. The statistics represent that programmers take a long time (several versions) to fix vulnerabilities in the Rust ecosystem.
%We obtained a total of 342 vulnerable packages (0.41\% of all packages in {\tt crates.io}), indicating that on average a vulnerable package had 2.28 vulnerabilities (the median was 2, the maximum was 18). 
%
\noindent\textbf{Overview of vulnerable packages.}
We identified a total of 337 vulnerable packages, accounting for 0.40\% of packages in the Rust ecosystem. 120 out of 337 vulnerable packages remain unpatched. The 337 vulnerable packages have an average of 1.3 disclosed vulnerabilities (min: 1, max: 14, median: 1, std: 1.04). The disclosed vulnerabilities affect an average of 28.6 versions of the Rust packages (min: 1, max: 339, median: 17, std: 34.33), accounting for 75.09\% of the versions per package on average (min: 1.37\%, max: 100\%, median: 82.07\%, std: 0.27). %The statistics represent that programmers take a long time (several versions) to fix vulnerabilities in the Rust ecosystem.
%
%\todo{[Jun 1] We would clarify the package that has the most vulnerabilities, as well as the package that has the most versions affected by vulnerabilities}\xy{[Jun 8] Done. }
%
% \todo{specify packages with maximum vulnerabilities, openssl-src, rusqlite}
% The top 5 packages with most vulnerabilities are \emph{openssl-src} (18 vulnerabilities, 95.45\% version, 42 versions affected), \emph{rusqlite} (17 vulnerabilities, 95.65\% version, 66 versions affected), \emph{hyper} (13 vulnerabilities, 96.27\% version, 207 versions affected), \emph{smallvec} (10 vulnerabilities, 72.45\% version, 37 versions affected) and \emph{ckb} (10 vulnerabilities, 36.00\% version, 9 versions affected). \emph{Rusqlite}, \emph{hyper} and \emph{smallvec} are popular packages in the Rust ecosystem as discussed in RQ1, suggesting that vulnerabilities are easier to exploit in popular packages. However, \emph{libc} with 100 million downloads and \emph{syn} with 111 million downloads have no vulnerability exploited, suggesting that officially published crates are highly secure. We also observe 114 vulnerable packages with all versions affected by vulnerabilities. There are 78 out of 114 vulnerable packages with less than 100,000 downloads over their time. This indicates that vulnerable packages with less popularity are prone to suffering from vulnerabilities for a long time and maintainers of the packages are inactive in fixing vulnerabilities.
%


The top 5 Rust packages with the most vulnerabilities are (1) {\tt openssl-src}, with 14 vulnerabilities and 55 versions affected (87.27\%), (2) {\tt wasmtime}, with 7 vulnerabilities and  62 versions affected (58.06\%), (3) {\tt hyper}, with 7 vulnerabilities and 224 versions affected (92.41\%), (4) {\tt ckb}, with 7 vulnerabilities and 32 versions affected (28.13\%), and (5) {\tt smallvec}, with 5 vulnerabilities and 54 versions affected (68.52\%). 
%
{\tt openssl-src}, {\tt hyper} and {\tt smallvec} are popular packages in the Rust ecosystem whose downloads are more than 9 millions in April 2023, suggesting that popular packages tend to have more vulnerabilities. \hl{One possible reason could be that popular packages have far more developers and users than less popular ones. The larger community of developers and users for popular Rust packages tend to uncover more vulnerabilities compared to less popular packages.} 
In contrast, some popular packages like {\tt libc} and {\tt syn}, which are officially published packages with over 100 million downloads, have no vulnerabilities disclosed, suggesting that officially published packages tend to be more secure.
%However, some popular but officially published packages, e.g., {\tt libc} and {\tt syn} with over 100 million downloads, has no vulnerabilities disclosed, suggesting that 
 We also observe that 109 vulnerable packages have all of their versions affected by vulnerabilities, out of which, 76 packages have less than 100,000 downloads in total over time. The observation indicates that less popular packages (with less than 100,000 downloads) tend to suffer from vulnerabilities for more versions. 



\begin{table}[!h]
%  \caption{Percentage of Rust crates with Vulnerabilities based on categories of crates.io.}
  \caption{Characteristics of packages in the Rust ecosystem.}
%  \todo{[Jun 1] The ``\# Crates'' and ``\# Downloads'' may be moved to RQ1, as a new table :-)}
%  \todo{[Jun 23] @Xiaoye, please double check the last row, in which the total of vulnerabilities is 814, not 776 :-)}\zy{[Jun 27] done.}
  \label{tab:category_percent}
  %\small
  \footnotesize
  \begin{tabular}{lcrrc}
    \toprule
%    Category    & \# Vulnerabilities &  \# Crates & \# Downloads & Vulnerabilities/Crates  \\
%    Vulnerable Category    & \# Vulnerabilities &  \# Crates & \# Downloads & Vulnerabilities/Crates  \\
%    Package Category    & \# Vulnerabilities &  \# Crates & \# Downloads & Vulnerabilities/Crates  \\
    \textbf{Package Category}    & \textbf{\# Vulnerabilities} &  \textbf{\# Packages} & \textbf{\# Downloads} & \textbf{Vulnerable Package \%}  \\
    \midrule
    Memory management       & 28    & 468       & 397,961,797       &5.98\%      \\
    Caching                 & 8    & 234     & 68,948,180           &3.42\%      \\
    Database interfaces     & 21    & 704       & 37,173,905        &2.98\%     \\
    Concurrency             & 26    & 909       & 799,571,861       &2.86\%      \\
    Data structures         & 54    & 2,144     & 1,170,205,196     &2.52\%     \\
    Network programming     & 33    & 2,138     & 816,412,017       &1.54\%     \\
    Asynchronous            & 28    & 1,900     & 1,039,591,569     &1.47\%     \\
    Encoding                & 22    & 1,494     & 904,623,837       &1.47\%     \\
    No standard library     & 50    & 3,671     & 3,704,866,624     &1.36\%     \\
    Rust patterns           & 15    & 1,158     & 829,299,334       &1.30\%     \\
    Parsing tools           & 16     & 1,272     & 363,898,651      &1.26\%     \\
    Text processing         & 11     & 943       & 484,155,024      &1.17\%    \\
    Cryptography            & 22    & 1,933     & 912,432,279       & 1.14\%   \\
    Web programming         & 27    & 2,386     & 650,382,813       & 1.13\%   \\
    Algorithms              & 17    & 1,595     & 1,190,075,755     &1.07\%     \\
    Web Assembly            & 8    & 921     & 197,555,288          &0.87\%     \\
    Multimedia              & 10     & 1,165     & 48,819,846       &0.86\%     \\
    Operating systems       & 8     & 1,013       & 603,471,887    &0.79\%     \\
    Science                 & 8    & 1,485     & 319,257,822        &0.54\%     \\
    API bindings            & 10     & 2,265     & 417,282,873      &0.44\%    \\
    Development tools       & 12    & 3,725     & 1,640,269,851     &0.32\%     \\
    Command line utilities  & 12    & 4,418     & 25,115,904        &0.27\%     \\
    (vulnerabilities<=6)   & 70 & 10,395   & 1,858,726,692 &0.67\%     \\
    \emph{Non-categorized}      & 214 & 55,895   & -              &0.38\%     \\
%    Total                           & 814    & 105,245    & -       & -     \\
    \bottomrule
  \end{tabular}
\end{table}



%and remain unpatched. 
%\todo{[Jun 21] @xiaoye, do we have any evidence for the following statement? If not, we may consider removing it:-)}\xy{most less popular packages remain unpatched. }% and maintainers of the packages are inactive in fixing vulnerabilities.

% \zy{Most popular package.}
% \emph{Rusqlite} package (around 4 million all-time downloads before May 1st, 2022) has 15 CVEs recorded in NVD, which are all related to memory safety issues. However, libc with 100 million downloads and syn with 111 million downloads have no vulnerability exploited, suggesting that these officially published crates are highly secure.

% \todo{[Jun 1] We would report the distribution of package categories of vulnerable packages:-)}
% Besides, we categorized vulnerabilities by the category of vulnerable package. On average, the number of package categories to which the vulnerable package belongs is 1.06 (median = 1). 166 vulnerable packages are not categorized by {\tt crates.io}. Excluding non-categorized packages, the average number of package categories to which the vulnerable package belongs is 2.09 (median = 2). 
%
%\autoref{tab:category_percent} reports the number of vulnerabilities in each package category, the total number of crates in the corresponding category, the total downloads of the category, and the vulnerabilities per crate. As the table shows, the top three categories with the highest number of absolute vulnerabilities are data structures, No standard library, and web programming. The categories of memory management, concurrency, and data structure have the top 3 vulnerabilities per crate. The category of memory management has a small number of crates (468) and downloads (397,961,797) compared to development tools and algorithms but has 54 vulnerabilities exploited so far. This result is somehow unexpected, which means that programmers are easy write vulnerabilities in memory management.


\noindent\textbf{Categories of Vulnerable Packages.}
We investigated the package categories of the 337 vulnerable packages. 165 vulnerable packages do not provide categorization information in {\tt crates.io}. For the rest 172 vulnerable packages, we identify an average of 2.10 package categories (median = 2). 
% finish above
For each package category, \autoref{tab:category_percent} reports the number of disclosed vulnerabilities, the number of packages, the number of downloads over time, and the average number of vulnerabilities per package. The top 3 package categories with the most vulnerabilities are \textit{data structures}, \textit{no standard library} and \textit{network programming}. In terms of the average number of vulnerabilities per package, \textit{memory management}, \textit{caching} and \textit{database interfaces} rank the top 3 among package categories. 
% finish above
Interestingly, the \textit{memory management} category has a smaller number of packages (468) with fewer downloads (397,961,797 downloads) compared with popular package categories but encounters a relatively larger number of vulnerabilities -- 28 vulnerabilities disclosed so far. The observation may suggest that developers tend to introduce vulnerabilities when dealing with memory management.

% \todo{[Jun 1] We would further report the distribution of vulnerability types across package categories of vulnerable packages :-)}
% We compared the distribution of vulnerability types across package categories of vulnerable packages. As \autoref{tab:cve_tpe_across_type} represents, \emph{memory management} category suffers from \emph{memory access}, \emph{memory mangement} and \emph{synchronization} vulnerability type most. The category of \emph{Concurrency} has \emph{synchronization} vulnerabilities most. \emph{Tainted Input} occurs most in the category of \emph{data structure} and \emph{network programming}.
%
%To check if the differences in the distribution of vulnerability types are statistically significant, we further employ the Wilcoxon signed-rank test\cite{wilcoxon} at 95\% significance level on 6 paired categories. In the 15 Wilcoxon signed-rank tests of the six categories, p-value between \emph{memory management} and \emph{data structures} is 0.02, p-value between \emph{caching} and \emph{data structures} is 0.003, p-value between \emph{caching} and \emph{no standard library} is 0.003, which means that the differences in the distribution of vulnerability types across these categories are significant.


%We further investigated the relationship between vulnerability types and package categories. Specifically, we compared the distribution of vulnerability types across the package categories with the highest vulnerable package percentages or most  vulnerabilities as shown in \autoref{tab:cve_tpe_across_type}.
We further investigated how package categories affect vulnerability types by comparing the distributions of vulnerability types across package categories.
Note that a vulnerability could have multiple vulnerability types. As shown in \autoref{tab:cve_tpe_across_type}, the packages in the \emph{memory management} category tend to suffer from \emph{memory access}, \emph{memory management} and \emph{synchronization} vulnerabilities; the packages in the \emph{concurrency} category encounters \emph{synchronization} and \emph{memory management} vulnerabilities most frequently; the \emph{tainted input} vulnerabilities occur most frequently in the packages of of the \emph{data structure} categories.
%
In addition, we investigated if the difference in the distributions of vulnerability types across package categories are statistically significant using the Wilcoxon signed-rank test~\cite{wilcoxon} \hl{with Bonferroni correction}
at 95\% significance level. We observe several statistically significant differences in the distributions: (1) \emph{caching} vs. \emph{data structures} \hl{(p-value = 0.0490)} and (2) \emph{caching} vs. \emph{no standard library} \hl{(p-value = 0.0490)}, indicating that package categories would significantly affect the disclosed vulnerability types in the Rust ecosystem.
%. The observation indicates that different categories of packages tend to suffer from different types of vulnerabilities, e.g., \emph{memory management} packages are prone to memory and synchronization issues.


\begin{table}[t]
  \caption{Vulnerability types in package categories in Rust.}
  %\todo{[Aug 8] There are 6 package categories in the table; which is also indicated in the corresponding paragraph; @Xiaoye, could you please help to confirm and fix the inconsistency?}\xy{Updated.}
  \label{tab:cve_tpe_across_type}
  \footnotesize
  % \tiny
%  \begin{tabular}{lp{0.8cm}p{0.8cm}p{0.8cm}p{0.6cm}p{0.8cm}p{0.8cm}}
%\begin{tabulary}{\textwidth}{lCCCCCC}
\begin{tabulary}{\textwidth}{lp{1.2cm}p{1.2cm}p{1.2cm}p{1cm}p{1.2cm}p{1.2cm}}
%\begin{tabulary}{\textwidth}{lCCCCCC}
    \toprule
     & \textbf{\scriptsize Memory Management} & \textbf{\scriptsize Concurrency} & \textbf{\scriptsize Data Structures} & \textbf{\scriptsize Caching} & \textbf{\scriptsize No Standard Library}&\textbf{\scriptsize Network Programming}\\
    \textbf{Vulnerability Type} & & & & & & \\
    \midrule
    Memory Access           & 11       & 8 & 19 & 2 & 25 & 11\\
    Memory Management       & 15       & 17 & 29 & 3 & 22 & 10\\
    Synchronization         & 10       & 17 & 11 & 4 & 8 & 4\\
    Tainted Input           & 2        & 4  & 5 & 0 & 1 & 3\\
    Resource Management     & 0        & 1  & 1 & 0 & 0 & 4\\
    Exception Management    & 1        & 0  & 4 & 0 & 4 & 3\\
    Cryptography            & 0        & 0  & 0 & 0 & 6 & 3\\
    Other                   & 0        & 0  & 3 & 0 & 4 & 2\\
    Risky Values            & 2        & 0  & 4 & 0 & 3 & 1\\
    Path Resolution         & 1        & 0  & 1 & 0 & 0 & 3\\
    % Information Leak        & 0        & 0  & 0 & 0 & 0\\
    % Privilege               & 0         & 0  & 0 & 0 & 0\\
    Predictability          & 0         & 0  & 0 & 0 & 2 & 0\\
    % Authentication          & 0         & 0  & 0 & 0 & 0\\
    API                     & 0         & 0  & 0 & 0 & 1 & 0\\
    % Access Control          & 0         & 0  & 0 & 0 & 0\\ 
    Failure to Release Memory & 0       & 0  & 1  & 0 & 0  & 0\\
    \emph{Total}                & 28    & 26 & 54 & 5 & 50 & 33\\
    \bottomrule
  \end{tabulary}
\end{table}

\begin{table}[t]
  \caption{Descriptive statistics of vulnerability locality.}
  \label{tab:vul_loc}
  \footnotesize
  \begin{tabular}{lcccc}
    \toprule
%    Descriptive Metrics & \# files & \# safe func & \# unsafe func & \# unsafe block \\
 & \textbf{\# Files} & \textbf{\# Safe Functions} & \textbf{\# Unsafe Functions} & \textbf{\# Unsafe Blocks} \\
    \midrule
    mean ($\mu$)    & 1.85  & 3.35  & 0.15  & 1.39\\
    median (M)      & 1     & 1     & 0     & 0\\
    min             & 1     & 0     & 0     & 0\\
    max             & 14    & 83    & 4    & 50\\
    std             & 1.95  & 8.84  & 0.53  & 5.20\\
    total           & -     & 684   & 31   & 284\\
    \bottomrule
  \end{tabular}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}

%

%\noindent\textbf{Vulnerability locations.}
%\noindent\textbf{Vulnerability locality.}
%\todo{[May 30] We may consider moving the part of ``vulnerability locality'' by analyzing vulnerable code in RQ2 :-) Note that, we could only focus on results of vulnerable code here:-)}
%\todo{[May 30] (1) affect how many files, (2) affect how many functions (safe and unsafe), and (3) affect how many unsafe blocks.}\xy{[Jun 12] Done.}
%
%We got 293 unique valid fix commits for 219 vulnerabilities in total. By investigating fix commits, we got statistic data of how many files, functions, and unsafe blocks vulnerabilities affect, as shown in \autoref{tab:vul_loc}. Note that a safe function may have unsafe blocks inside its function body. We observe that around 85\% vulnerable functions are safe functions and around 26.9\% vulnerable safe functions have an unsafe block in the function bodies. Therefore, most vulnerabilities exist in safe functions. 
\begin{figure}[t]
\centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=6.5cm]{sections/fig/func_distribution.pdf}
        \caption{\hl{Ratios of unsafe functions in vulnerable code vs. all code of vulnerable packages.}}
        %\todo{[Jun 1] the x axis would be consistent with that of \autoref{fig:numVulnerability}}
        \label{fig:disFunc}
    \end{minipage}
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=7cm]{sections/fig/block_distribution.pdf}
        \caption{\hl{Ratios of unsafe blocks  in vulnerable code vs. all code of vulnerable packages.}}
        %\todo{[Jun 1] the x axis would be consistent with that of \autoref{fig:numVulnerability}}
        \label{fig:disBlock}
    \end{minipage}
\end{figure}

\noindent\textbf{Vulnerability locality in vulnerable packages.} 
% We quantified the impact of a vulnerability in the Rust ecosystem by its locality, i.e., the number of files, functions, and unsafe blocks the vulnerability affected. 
 %\hl{the vulnerable code versions on average contains 637.22 safe functions, 16.69 unsafe functions and 77.30 unsafe blocks (226 safe functions, 2 unsafe functions, 14 unsafe blocks in median) in total. Specifically, we used Wilcoxon signed-rank test at 95\% significance level to investigate if the difference between vulnerable packages and vulnerability locality in the distributions of the percentage of unsafe functions (the number of unsafe functions divided by the number of total functions) /unsafe blocks (the number of unsafe blocks divided by the number of safe functions) are statistically significant. We observe statistically significant differences in both percentage of unsafe functions and unsafe blocks: (1) vulnerable packages vs. vulnerability locality in the percentage of unsafe functions (p-value = 0.002); (2) vulnerable packages vs. vulnerability locality in the percentage of unsafe blocks (p-value = 0.017). The observation indicates that the vulnerable code could involve more unsafe code.} The distributions of the percentage of unsafe functions and unsafe blocks in vulnerability locality and vulnerable packages are shown in \autoref{fig:disFunc} and \autoref{fig:disBlock}.
As illustrated in \autoref{tab:vul_loc},\hl{ a disclosed vulnerability affects 1.85 files, 3.35 safe functions, 0.15 unsafe functions, and 1.39 unsafe blocks in the vulnerable packages in the Rust ecosystem on average (1 file, 1 safe function, 0 unsafe function, and 0 unsafe block in median)}. \hl{The median number of files associated with vulnerable code is just one, while the highest number of affected files within a single commit is 14, indicating that vulnerable code tends to be relatively small.} \hl{95\% of the functions affected are safe functions, and 41.5\% of the safe functions affected contain unsafe blocks in their body of a function. One possible reason for the high percentage of safe functions in vulnerable code is that developers tend to wrap unsafe code in safe functions and provide conditional checks in those functions before entering the unsafe code.} 
%As shown in \autoref{tab:total_loc}, \hl{the vulnerable packages contain an average of 637.22 safe functions, 16.69 unsafe functions and 77.30 unsafe blocks (a median of 226 safe functions, 2 unsafe functions, and 14 unsafe blocks). } 
%\autoref{fig:disFunc} and \autoref{fig:disBlock} \hl{present the ratios of unsafe functions and blocks in vulnerable code and all code of vulnerable packages, respectively.} 

\hl{We compared the ratios of unsafe functions and blocks between vulnerable code and all code in vulnerable packages as shown in} \autoref{fig:disFunc} and \autoref{fig:disBlock}. 
\hl{Vulnerable code shows higher ratios of both unsafe functions and unsafe blocks compared to all code in vulnerable packages. In vulnerable code, the average ratio of unsafe functions and unsafe blocks are 0.059 and 0.261, respectively, which are higher compared to all code for unsafe functions (0.034) and unsafe blocks (0.165). The median ratio of unsafe functions in vulnerable code is 0, while in all code it is 0.003. The median ratio of unsafe blocks in vulnerable code is 0, while in all code it is 0.086. 
%
The Wilcoxon signed-rank test at 95\% significance level indicates that vulnerable code in vulnerable packages tends to involve more unsafe functions (p-value = 0.002) and more unsafe blocks (p-value = 0.017).}
% We compared the ratios of unsafe functions and blocks between vulnerable code and all code in vulnerable packages using the Wilcoxon signed-rank test at 95\% significance level. The results indicate that vulnerable code tends to involve more unsafe functions (p-value = 0.002) and more unsafe blocks (p-value = 0.017).}
 



\begin{table}[t]
\caption{Statistics of vulnerability locality across vulnerability types.} %(M: Mean, Mdn: Median, \#C: the number of commits)}
  \label{tab:fun_cnt_across_type}
  %\footnotesize
  \tiny
\begin{tabular}{lllllllll}
%\hline
\toprule
\multicolumn{2}{l}{\textbf{Vulnerability type}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Memory \\ Access\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Memory \\ Management\end{tabular}} &
  \textbf{Synchronization} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Tainted \\ Input\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Resource \\ Management\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Exception \\ Management\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Path \\ Resolution\end{tabular}}\\% \hline
 \midrule
\multicolumn{2}{l}{\textbf{\# Commits}}                                   & 42    & 28   & 39   & 21    & 9   & 6   & 6\\ \midrule
\multicolumn{1}{l}{\multirow{5}{*}{\textbf{\# Files}}}            & $\mu$ & 2.30  & 2.14 & 1.59 & 1.57  & 1.89& 2.33& 1.83 \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & M     & 1     & 1    & 1    & 1     & 2    & 2  & 1.5 \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & min   & 1     & 1    & 1    & 1     & 1    & 1  & 1 \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & max   & 14    & 14   & 5    & 4     & 3    & 5  & 3\\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & std   & 2.94  & 2.72 & 1.25 & 0.95  & 0.93 & 1.51 & 0.98\\ \midrule
\multicolumn{1}{l}{\multirow{5}{*}{\textbf{\# Safe functions}}}   & $\mu$ & 3.88  & 4.32 & 1.05 & 1.43  & 2 & 8.67 & 1.33\\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & M     & 1     & 1    & 0    & 1     & 2    & 3    & 1\\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & min   & 0     & 0    & 0    & 0     & 1    & 1    & 1\\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & max   & 59   & 33   & 13   & 5     & 5   & 40    & 3\\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & std   & 10.92 & 8.56 & 2.67 & 1.12  & 1.32 & 15.41 & 0.82\\ \midrule
\multicolumn{1}{l}{\multirow{5}{*}{\textbf{\# Unsafe functions}}} & $\mu$ & 0.17  & 0.14 & 0.15 & 0.05  & 0   & 0 & 0\\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & M     & 0     & 0    & 0    & 0     & 0    & 0   & 0 \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & min   & 0     & 0    & 0    & 0     & 0    & 0   & 0 \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & max   & 2    & 3    & 2   & 1     & 0    & 0   & 0 \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & std   & 0.44  & 0.59 & 0.49 & 0.22  & 0    & 0 & 0\\ \midrule
\multicolumn{1}{l}{\multirow{5}{*}{\textbf{\# Unsafe blocks}}}    & $\mu$ & 2.14  & 2.39 & 0.21 & 0.19  & 0 & 7.67 & 0\\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & M     & 0     & 0    & 0    & 0     & 0    & 2  & 0  \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & min   & 0     & 0    & 0    & 0     & 0    & 0   & 0 \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & max   & 50    & 67    & 6   & 3     & 0    & 40   & 0 \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & std   & 7.85  & 6.32 & 0.98 & 0.68  & 0 & 15.87 & 0\\
\bottomrule
\end{tabular}
\end{table}

%
%Furthermore, we study the statistical data across vulnerability types. \autoref{tab:fun_cnt_across_type} represents that memory management vulnerabilities locate both in the safe functions and unsafe functions. Vulnerabilities in the type of \emph{memory access} are mostly located in the safe function and involve around 5 safe functions on average, which are far more than the number of safe functions in other types. This indicates that vulnerable code in \emph{memory access} exists in a large range of functions. Synchronization vulnerabilities are mostly located in unsafe code (including unsafe functions and unsafe blocks). The average number of safe functions in \emph{Synchronization} is 1.37 and the average number of unsafe blocks in \emph{Synchronization} is 1.30, which means, on average, each safe function contains an unsafe block inside the function body. \emph{Tainted input} and \emph{resource management} vulnerabilities are mostly located in safe code and the vulnerable code is hardly in the unsafe blocks. 

%Furthermore, we investigated the differences in vulnerability locality across vulnerability types. As \autoref{tab:fun_cnt_across_type} illustrated, the \textit{memory management} vulnerabilities tend to locate in both the safe and unsafe functions. The \emph{memory access} vulnerabilities tend to mainly occur in safe functions, involving an average of 5 safe functions. The average number of safe functions involved in the \emph{memory access} vulnerabilities is far greater than that of other types of vulnerabilities, indicating that \emph{memory access} vulnerability-related code is less localized across functions compared to other types of vulnerabilities. The \textit{synchronization} vulnerabilities tend to locate in unsafe functions and unsafe blocks, involving an average of 1.59 
%\todo{[Jun 21] 1.59? as shown in the table.}\xy{Updated.} 
%safe functions and 1.30 unsafe blocks. On average, one safe function involved in \textit{synchronization} vulnerabilities contains an unsafe block inside its function body.
% Furthermore, we investigated the differences in vulnerability locality across vulnerability types. 
% We further investigated how vulnerability types affect the locality of vulnerable code by comparing the numbers of safe functions and unsafe blocks in vulnerable code across vulnerability types. 
\autoref{tab:fun_cnt_across_type} presents the comparison results of vulnerability localities across vulnerability types in terms of numbers of commits, files, safe and unsafe functions, and unsafe blocks. The \emph{memory management} and \emph{memory access} \hl{vulnerabilities tend to locate in safe functions half of whose body has unsafe blocks. We observed that 77\% vulnerabilities of memory safety and concurrency involve unsafe code. The average number of safe functions and unsafe blocks involved in the} \emph{exception management} \hl{vulnerabilities is far greater than that of other types of vulnerabilities, indicating that }\emph{exception management} \hl{vulnerability-related code is less localized and involves more codes compared to other types of vulnerabilities.} The \emph{synchronization} vulnerabilities tend to locate in an average of 1 safe function (median = 0). Note that \emph{synchronization} vulnerabilities involve an average of 1 unsafe trait or trait implement (median = 1).
%
Most of the \emph{tainted input}, \emph{resource management} and \emph{path resolution} vulnerabilities originate from safe code;  the corresponding vulnerable code is rarely located in unsafe blocks.


%\vspace{-0.1cm}
\begin{tcolorbox}[width=\linewidth,
                  boxrule=0.5pt,
                  arc=0mm,
                  left=0pt,
                  right=0pt,
                  top=2pt,
                  colback=yellow!30]

\textbf{Summary for RQ2:} 
%We observe that popular packages tend to be targets of attack and less popular packages tend to suffer from vulnerabilities for more versions. In addition, around 85\% vulnerable functions are safe functions and 26.9\% of the safe functions affected contain unsafe blocks in their body of the function.

% The top 5 Rust packages with the most vulnerabilities are (1) {\tt openssl-src}, with 18 vulnerabilities and 95\% versions affected, (2) {\tt rusqlite}, with 17 vulnerabilities and 96\% versions affected, (3) {\tt hyper}, with 13 vulnerabilities and 96\% versions affected, (4) {\tt smallvec}, with 10 vulnerabilities and 72\% versions affected, and (5) {\tt ckb}, with 10 vulnerabilities and 36\% versions affected. 
%
The more popular packages tend to suffer from more vulnerabilities, while the less popular packages tend to suffer from vulnerabilities for more versions. 
%
\emph{memory management} is the most vulnerable package category with relatively small number of packages while large number of vulnerabilities. 
Different categories of packages tend to suffer from different types of vulnerabilities.
%
The average ratio of unsafe functions (0.059) and unsafe blocks (0.261) in vulnerable code are higher compared to all code in vulnerable packages for unsafe functions (0.034) and unsafe blocks (0.165), which suggests that vulnerable code tends to involve more unsafe code.
\end{tcolorbox}

% \zy{OLD.}
% \autoref{tab:decript_unsafe} shows the main descriptive statistics on the number of modified safe/unsafe functions and blocks before and after the fix commit. We found that the sum of unsafe functions in all vulnerabilities takes 53.05\% and the sum of unsafe blocks in all vulnerabilities takes 50.74\%. Around half of the functions related to vulnerabilities are safe functions, which means safe code is not truly safe. In total, the sum of safe functions is less than unsafe functions. We found that the median of the number of unsafe functions related to the vulnerability is 1 and the median of the number of safe functions related to the vulnerability is 0.  We can imply that safe code could avoid some vulnerabilities to some extent. The data of the two-level analysis is consistent and suggests that both unsafe code and safe code cause vulnerabilities in the Rust library, but unsafe code leads to slightly more vulnerabilities than safe code.

% \todo{[MOST IMPORTANT][Jun 1] We have two versions for ``Types of vulnerabilities'' and ``Vulnerable Rust packages'' currently, ABOVE and BELOW; which version is based on our new methodology and dataset?}

%\noindent\textbf{Types of vulnerabilities.}
%\autoref{tab:cve_tpe} presents the distribution of vulnerabilities over vulnerability types described by Rustsec. We could see that the two-fifths of vulnerabilities are not classified by Rustsec. Excluding those not classified vulnerabilities, We can observe that the top three vulnerability types are memory-corruption (26.64\%), thread safety (11.00\%), and memory-exposure (7.92\%). Privilege-escalation (0.58\%) and file-disclosure (0.97\%) are rare in Rust related vulnerabilities. Memory safety issues and concurrency problems account for almost half of all the categorized vulnerabilities, suggesting that Rust still cannot avoid memory issues in practice.  

%When analyzing the type of disclosed vulnerabilities in detail, we observe that almost 30\% of the advisories come from a large-scale campaign and not a broader community effort: there are 129 memory safety and soundness vulnerabilities disclosed as part of the research efforts of Yechan Bae\cite{Rudra}. Nevertheless, this shows the feasibility of large-scale vulnerability detection and reporting on Rust.

% \noindent\textbf{Vulnerable Rust packages.}
% We found most Rust libraries have no vulnerabilities, as \autoref{tab:lib_cve} shows. Only 288 libraries (corresponding to the 0.36\%) have one or more vulnerabilities discovered by now, but there are 80,268 Rust libraries in total. 
%
% In particular, 205 crates in 288 vulnerable crates have only one vulnerability discovered so far. 
%
\par


% \todo{[Apr 28] For each table, we would introduce what each column represents first:-)}


% \begin{table}[t]
%   \caption{The Count and Percentage of Libraries That Have and Have No Vulnerabilities}
%   \todo{[Jun 1] We may consider remove this table; we would just report the number of vulnerable packages in the Rust ecosystem.}
%   \label{tab:lib_cve}
%   \begin{tabular}{ccl}
%     \toprule
%     Vulnerabilities &Libraries & Percentage \\
%     \midrule
%     0 & 79,980 & 99.64\% \\
%     > 0 & 288 & 0.36\% \\
%     In total & 80,268 & 100.00\% \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\begin{table}[t]
  %\caption{Summary of descriptive statistics of Commit Locality}
  \caption{\hl{Descriptive statistics of vulnerability fixes.}}
  \label{tab:commit_loc}
  %\small
  \footnotesize
%  \begin{tabular}{lp{0.8cm}p{0.8cm}p{1.5cm}p{1.5cm}p{1cm}}
\begin{tabular}{lcc|ccc}
    \toprule
    %Descriptive Metrics & \# lines added & \# lines deleted & \# safe func & \# unsafe func & \# unsafe block \\
     & \textbf{\# Lines Added} & \textbf{\# Lines Deleted} & \textbf{\# Safe Functions} & \textbf{\# Unsafe Functions} & \textbf{\# Unsafe Blocks} \\
    \midrule
    mean ($\mu$)    & 41.13     & 18.17      & 3.85  & 0.16  & 1.49\\
    median (M)      & 14        & 4          & 1     & 0     & 0\\
    min             & 1         & 0          & 0     & 0     & 0\\
    max             & 665       & 330        & 83    & 4    & 50\\
    std             & 81.97     & 39.75      & 9.12  & 0.53  & 5.24\\
    total           & -         & -          & 786   & 32   & 304\\
    \bottomrule
  \end{tabular}
\end{table}


%\subsection{RQ3: Library Risk Analysis}
%\subsection{RQ3: Locations and Fixes of Rust Vulnerabilities}
%\subsection{RQ3: Vulnerability Fixes in the Rust Ecosystem}
\subsection{RQ3: Vulnerability Fixes in the Rust Ecosystem}
% \noindent\textbf{Vulnerability locations.}
% \autoref{tab:decript_unsafe} shows the main descriptive statistics on the number of modified safe/unsafe functions and blocks before and after the fix commit. We found that the sum of unsafe functions in all vulnerabilities takes 53.05\% and the sum of unsafe blocks in all vulnerabilities takes 50.74\%. Around half of the functions related to vulnerabilities are safe functions, which means safe code is not truly safe. In total, the sum of safe functions is less than unsafe functions. We found that the median of the number of unsafe functions related to the vulnerability is 1 and the median of the number of safe functions related to the vulnerability is 0.  We can imply that safe code could avoid some vulnerabilities to some extent. The data of the two-level analysis is consistent and suggests that both unsafe code and safe code cause vulnerabilities in the Rust library, but unsafe code leads to slightly more vulnerabilities than safe code.
% \todo{[May 30] We will focus RQ3 on characteristics of vulnerability fixes:-)}
%
% \todo{[May 30] This is similar to vulnerability locality in RQ2; the difference is that we would consider ``removed'' and ``added'' lines together, i.e., vulnerable and fixing code together :-) (1) affect how many files, (2) affect how many functions (safe and unsafe), (3) affect how many unsafe blocks.}\xy{[Jun 12] Done.}
% \noindent\textbf{Commit complexity.}
% Given the diversity of software projects we consider, we chose lines of code (LOC) as a simple-albeit-rudimentary metric to assess commit complexity, as with prior studies~\cite{ccs2017-18,ccs2017-26,SZZ,ccs2017-41}. From \autoref{tab:commit_loc}, we could find that the median fix commits diff involved 15 LOC added and 5 LOC deleted. From this perspective, we could infer that programmers prefer to add lines to fix the vulnerabilities in the Rust ecosystem.
% \noindent\textbf{Commit locality.}
%We got descriptive statistic data of functions and unsafe blocks in fixing commit, as shown in \autoref{tab:commit_loc}. Note that we counted both functions in vulnerable code and functions in fixing code. We observe that around 86.6\% fixing involved functions are safe functions and around 22.3\% fixing involved safe functions have an unsafe block in the function bodies in total. Comparing \autoref{tab:commit_loc} and \autoref{tab:vul_loc}, the number of safe functions increases, suggesting that maintainers fix vulnerabilities by adding safe functions or adding lines in safe functions. The slight increase of unsafe functions and blocks indicates that programmers need to add unsafe code to fix the vulnerability sometimes.
\noindent\textbf{Fix commit complexity and locality.}
% We characterized the fixes of disclosed vulnerabilities in the Rust ecosystem, in terms of the complexity of vulnerability fixes and locality of relevant code changes. 
%
As shown in \autoref{tab:commit_loc}, the commits of vulnerability fixes involve \hl{an average of 41 LOC added and 18 LOC deleted (median: 14 added, 4 deleted). The fix commits touched 3.85 safe functions, 0.16 unsafe functions, and 1.49 unsafe blocks on average. 96\% of the functions touched by vulnerability fix commits are safe functions, among which 38.8\% contain unsafe blocks.}.
%
% \todo{[May 18] We would further compare the locations for different types of vulnerabilities :-)}
% \autoref{tab:commit_fun_cnt_across_type} shows the statistic data of fixing code across vulnerability types, similar to \autoref{tab:fun_cnt_across_type}. Together with \autoref{tab:commit_fun_cnt_across_type} and \autoref{tab:fun_cnt_across_type}, we can observe that in the category of \emph{memory access}, the number of safe functions and unsafe functions increase drastically, which indicates that programmers fix vulnerabilities by adding safe functions and unsafe functions. In the category of \emph{synchronization}, the statistics are similar to the code before fix commit, suggesting that programmers modify the code or remove some code to fix vulnerabilities. In the category of \emph{resource management} and \emph{tainted input}, adding safe functions or adding lines in safe functions is the popular choice. In \emph{exception management}, programmers fix the vulnerabilities by modifying the vulnerable code in place.
% Next, we explored the commit locality of vulnerability fixes across vulnerability types. \autoref{tab:commit_fun_cnt_across_type} illustrates the statistics of vulnerability fixes across vulnerability types, in terms of the number of safe functions, unsafe functions, and unsafe blocks touched by fixes. Fixes for the \emph{memory access} vulnerabilities involve an average of 4 safe functions, which is more than the number of safe functions involved in the fixes of other types of vulnerabilities. We observe an addition of 1 safe functions on average (2.17 vs. 1.33 in \autoref{tab:vul_loc}) for fixing \emph{path resolution} vulnerabilities.
Next, we explored the commit locality of fix commits across vulnerability types. \autoref{tab:commit_fun_cnt_across_type} illustrates the statistics of vulnerability fix commits across vulnerability types, in terms of the number of safe functions, unsafe functions, and unsafe blocks touched by commits. The fix commits of \emph{exception management} vulnerabilities involve the most safe functions (an average of eight) compared to other types of vulnerabilities, indicating potential challenges of fixing \emph{exception management} vulnerabilities in practice. Compared to \autoref{tab:fun_cnt_across_type}, fix commits for the \emph{memory access} \hl{vulnerabilities involve an average of 4 safe functions (median: 1) and an average of 2.17 unsafe blocks (median: 0), which indicates that more safe functions and unsafe blocks are added or modified in fix commits. We observe an addition of 1 safe functions on average (2.17 vs. 1.33 in} \autoref{tab:fun_cnt_across_type}) for fixing \emph{path resolution} vulnerabilities.

%\noindent\textbf{Fix patterns.} \todo{[May 30] We could refer to ICSME 2017 repeated bug fixes.}
% We randomly selected xxx commits from various locations of each vulnerability type and further conducted the manual inspection. 


% Table generated by Excel2LaTeX from sheet 'Sheet1'

\begin{table}[t]
\caption{Statistics of commit locality of vulnerability fixes across vulnerability types.} %(M: Mean, Mdn: Median, \#C: the number of commits)}
  \label{tab:commit_fun_cnt_across_type}
  \tiny
\begin{tabular}{lllllllll}
% \hline
\toprule
\multicolumn{2}{l}{\textbf{Vulnerability Type}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Memory \\ Access\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Memory \\ Management\end{tabular}} &
  \textbf{Synchronization} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Tainted \\ Input\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Resource \\ Management\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Exception \\ Management\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Path \\ Resolution\end{tabular}}\\% \hline
 \midrule
\multicolumn{2}{l}{\textbf{\# Commits}}                                   & 42    & 28   & 39   & 21   & 9    & 6       & 6   \\ \midrule
\multicolumn{1}{l}{\multirow{5}{*}{\textbf{\# Safe Functions}}}   & $\mu$ & 4.0   & 4.71 & 1.21 & 2.0  & 3.44 & 8.67    &2.17\\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & M     & 1     & 2    & 0    & 1    & 2    & 3       & 2 \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & min   & 0     & 0    & 0    & 0    & 1    & 1       &1 \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & max   & 59    & 33   & 16   & 8    & 12   & 40      &5\\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & std   & 10.89 & 8.60 & 3.22 & 1.79 & 3.50 & 15.41   & 1.47\\ \midrule
\multicolumn{1}{l}{\multirow{5}{*}{\textbf{\# Unsafe Functions}}} & $\mu$ & 0.19  & 0.14 & 0.15 & 0.05 & 0    & 0       & 0\\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & M     & 0     & 0    & 0    & 0    & 0    & 0       & 0   \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & min   & 0     & 0    & 0    & 0    & 0    & 0       & 0   \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & max   & 2     & 3    & 2    & 1    & 0    & 0       & 0 \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & std   & 0.45  & 0.59 & 0.49 & 0.22 & 0    & 0       & 0\\ \midrule
\multicolumn{1}{l}{\multirow{5}{*}{\textbf{\# Unsafe Blocks}}}    & $\mu$ & 2.17  & 2.39 & 0.21 & 0.24 & 0    & 7.67    & 0 \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & M     & 0     & 0    & 0    & 0    & 0    & 2       & 0  \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & min   & 0     & 0    & 0    & 0    & 0    & 0       & 0  \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & max   & 50    & 33   & 6    & 3    & 0    & 40      & 0  \\ %\cline{2-8} 
\multicolumn{1}{l}{}                                              & std   & 7.84  & 6.32 & 0.98 & 0.70 & 0    & 15.87   & 0\\ 
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
  \centering
  %\caption{Vulnerability fix patterns.}
  \caption{The characteristics of vulnerability fix commits across localities.}
%  \todo{[May 30] to be updated.}
  \footnotesize
    \begin{tabular}{p{0.5cm}lr}
    \toprule
    \multicolumn{1}{c}{\textbf{Vulnerability Locality}} & \multicolumn{1}{l}{\textbf{Fix Pattern}} & \multicolumn{1}{c}{\textbf{Count}} \\
    \midrule
    \multicolumn{1}{l}{Safe function} & add safe functions & 28 \\
          & remove safe functions &  12 \\
          & modify safe functions & 117 \\
    \midrule
    \multicolumn{1}{l}{Unsafe function} & add unsafe functions &  0\\
          & remove unsafe functions & 0 \\
          & modify unsafe functions & 16 \\
    \midrule
    \multicolumn{1}{l}{Unsafe block} & add functions or lines in function & 5 \\
          & remove unsafe blocks &  27\\
          & modify unsafe blocks &  36\\
    \bottomrule
    \end{tabular}%
  \label{tab:fix_pattern}%
\end{table}%

\noindent\textbf{Vulnerability fix patterns.}
To capture how developers fix vulnerabilities, we further analyzed the vulnerability fixes across vulnerabilities with different localities. As discussed in \autoref{sec:result_RQ2}, vulnerabilities in vulnerable packages locate in safe functions, unsafe functions and unsafe blocks, thus we summarized the fix patterns with respect to different vulnerability localities as shown in \autoref{tab:fix_pattern}. 
In general, three operations involved when developers apply fixes, \emph{addition}, \emph{deletion}, and \emph{modification} of code. Modification of code accounts for the majority of vulnerability fix commits with different localities. In our manual inspection, we made the following observations:

% To better understand the vulnerability fixing approach, we analyze the fix commits in detail. We consider the vulnerable code located only in safe functions as safe functions vulnerability locality, the vulnerable code located only in unsafe functions as unsafe function vulnerability locality, and the vulnerable code located in unsafe blocks as an unsafe block. 
% Note that a vulnerable code may have lots of vulnerability locality. From \autoref{tab:fix_pattern}, we observe that most of the vulnerabilities are fixed by modifying the code in place. 

%Programmers like to add safe functions or lines in safe functions to fix the vulnerable safe functions. This result indicates that programmers prefer to insert new code rather than remove existing code to fix the bug in Rust crates.Take GHSA-m5pq-gvj9-9vr8 vulnerability as an example, the fix commit ae70b fixes the \emph{denial-of-service} bug. As shown in \autoref{lst:add_func_example}, the fix adds another function {\tt c\_empty()} to deal with the empty string which may cause denial-of-service bug.
% \todo{[Jun 21] @xiaoye, please confirm if my rephrased description about the example fixes of 3 observations are correct and precise:-)}

\noindent\textbf{Observation 1: Developers \hl{tend to} add safe functions, or add lines in safe functions to fix vulnerable safe functions.} The observation indicates that developers tend to insert new code, rather than remove existing code to fix vulnerabilities in vulnerable code that involve safe functions. \hl{Through manual inspection of vulnerability fixes, we find that the added safe functions intend to validate pre-conditions or customize the default implemented functions to prevent potential vulnerabilities.}
Taking the fix of the \emph{denial-of-service} vulnerability (CVE-2022-24713) %(\todo{[Jun 21] what does the GHSAxx string mean?  CVE-2022-24713? } \xy{GHSAxx is the GitHub Advisory ID. GHSA-m5pq-gvj9-9vr8 and CVE-2022-24713 is the same vulnerabilitiy.} GHSA-m5pq-gvj9-9vr8) 
as an example, the fix inserts an additional function {\tt c\_empty()} to deal with the empty string which may cause denial of service, as shown in \autoref{lst:add_func_example}.




%\begin{lstlisting}[caption={Adding function when fix the vulnerability},label={lst:add_func_example},language=Rust]
\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Example vulnerability fix ( CVE-2022-24713).},label={lst:add_func_example},language=Rust,basicstyle=\small\ttfamily]
// code snapshot before fix commit
fn c(&mut self, expr: &Hir) -> ResultOrEmpty {
    ...
    match *expr.kind() {
        Empty => Ok(None),
        ...
    }
}
    
// code snapshot after fix commit
fn c_empty(&mut self) -> ResultOrEmpty {
    self.extra_inst_bytes += 
        std::mem::size_of::<Inst>();
    Ok(None)
}
fn c(&mut self, expr: &Hir) -> ResultOrEmpty {
    ...
    match *expr.kind() {
        Empty => self.c_empty(),
        ...
    }
}

\end{lstlisting}
\end{minipage}

%When a vulnerability lies in an unsafe block, removing unsafe blocks rather than adding functions is a popular way to fix the vulnerability. Take RUSTSEC-2021-0086 as an example, the vulnerability reads from uninitialized memory, which could produce undefined values that can quickly invoke undefined behavior. The fix commit for the vulnerability is 1b643d. In the commit, programmers ensure the buffer is zeroed for reading and remove the unsafe block in the code, as shown in \autoref{lst:remove_unsafe}.

\noindent\textbf{Observation 2: Developers tend to remove unsafe blocks to fix vulnerable unsafe blocks.}  The observation indicates that developers tend to remove existing code, rather than insert new code to fix vulnerabilities that involve unsafe blocks. Taking the fix of the memory exposure vulnerability (RUSTSEC-2021-0086) as an example, the fix ensures the buffer is flushed before further reading and removes the unsafe block in the vulnerable code, as shown in \autoref{lst:remove_unsafe}.

% \begin{lstlisting}[caption={Removing unsafe code when fix the vulnerability},label={lst:remove_unsafe},language=Rust]
\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Example vulnerability fix ( RUSTSEC-2021-0086).},label={lst:remove_unsafe},language=Rust,basicstyle=\small\ttfamily]
// code snapshot before fix commit
let mut buf = Vec::with_capacity(frame.data_size);
unsafe { buf.set_len(frame.data_size) };
    
// code snapshot after fix commit
let mut buf = vec![0; frame.data_size];
\end{lstlisting}
\end{minipage}

%Besides, in the unsafe function vulnerability locality, we find a vulnerability pattern about data race: Objects are not restricted to Send able types or Sync able types when they implement Send or Sync trait, which leads to non-Sync types shared across threads in concurrent programs, as shown in \autoref{lst:send_sync}. There are 31 vulnerabilities caused by this pattern and fixed by modifying unsafe trait implements.
\noindent\textbf{Observation 3: Developers tend to modify unsafe trait implements to fix vulnerable unsafe functions.} In terms of vulnerabilities located in unsafe traits, we identified a \textit{data race} vulnerability pattern from 31 disclosed vulnerabilities. Specifically, objects do not restrict to sendable types or syncable types when they implement {\tt Send} or {\tt Sync} trait, leading to non-syncable types shared across threads in concurrent Rust programs, as shown in \autoref{lst:send_sync}. 

%\begin{lstlisting}[caption={Send/Sync implementation},label={lst:send_sync},language=Rust]
\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Example vulnerability fix involving {\tt Send}/{\tt Sync}  implementation.},label={lst:send_sync},language=Rust,basicstyle=\small\ttfamily]
// code snapshot before fix commit
unsafe impl<T> Send for MyObject<T> {}
unsafe impl<T> Sync for MyObject<T> {}
    
// code snapshot after fix commit
unsafe impl<T: Send> Send for MyObject<T> {}
unsafe impl<T: Send> Sync for MyObject<T> {}
\end{lstlisting}
\end{minipage}


\begin{tcolorbox}[width=\linewidth,
                  boxrule=0.5pt,
                  arc=0mm,
                  left=0pt,
                  right=0pt,
                  top=2pt,
                  colback=yellow!30]


\textbf{Summary for RQ3:} 
%Vulnerability fixes involve an average of 49 LOC added and 26 LOC deleted, and reside in 4.15 safe functions, 0.65 unsafe functions, and 0.92 unsafe blocks on average. Furthermore, we find three major observations of fix commits: 1) Developers tend to add safe functions or add lines in safe functions to fix vulnerable safe functions; 2) Developers tend to remove unsafe blocks to fix vulnerabilities located in unsafe blocks; 3) Developers tend to modify unsafe trait implements to fix vulnerabilities located in unsafe functions.

Vulnerability fix commits in the Rust ecosystem involve a median of 14 lines of code added, and 4 lines of code deleted. The fix commits touch an average of 3.85 safe functions, 0.16 unsafe functions, and 1.49 unsafe blocks on average.
%
% Safe functions account for a majority of the functions involved in the vulnerability fixes (96\%). 
96\% of the functions touched by fix commits are safe functions.
%
The fix commits of \emph{exception management} vulnerabilities involve the most safe functions (an average of eight) compared to other types of vulnerabilities, indicating potential challenges of fixing \emph{exception management} vulnerabilities in practice.
%
In addition, developers tend to (1) add safe functions or add lines in safe functions to fix vulnerable safe functions, (2) remove unsafe blocks to fix vulnerable unsafe blocks, and (3) modify unsafe trait implements to fix vulnerable unsafe functions.

\end{tcolorbox}
% We find two fix patterns and one vulnerability pattern when scrutiny the code and fix commits. 45 (15.36\%) fix commits add other functions or only add lines in functions but not modify or delete any code in functions when fixing the vulnerabilities. However, only 29 (9.90\%) fix commits remove functions or only delete lines in functions. This result indicates that programmers prefer to insert new code rather than remove existing code to fix the bug in Rust crates. We also observe that 28 (9.55\%) fix commits remove at least one unsafe function or unsafe block to fix the vulnerabilities.  Besides, we find a vulnerability pattern about data race: Objects are not restricted to Send able types or Sync able types when they implement Send or Sync trait, which leads to non-Sync types shared across threads in concurrent programs, as shown in \autoref{lst:send_sync}. There are 31 (14.16\%) vulnerabilities caused by this pattern. 




% \zy{OLD version below; consider to remove :-)}\noindent\textbf{Characteristics of vulnerability fixes.}
% \zy{What statistics do we plot exactly?}
% \autoref{fig:violinPlot} presents violin plots that show the distribution of modified or deleted safe/unsafe functions and blocks before fix commit, as well as modified or added safe/unsafe functions and blocks after fix commit, for all vulnerabilities that have public fix commit. The width of each violin corresponds to the frequency of vulnerabilities with that number.  We filtered out vulnerabilities that have more than 10 blocks or functions which is rare, for better representation in the violin plot. 

% \zy{So, the violin plots give the same stats as Table~\ref{tab:decript_unsafe}?}
% Together with \autoref{tab:decript_unsafe} and \autoref{fig:violinPlot}, we can observe that both at the function level and block level, the number of safe code increase after fix commit, which means that programmers add safe code to fix vulnerabilities. The number of unsafe functions before the fix commit is more than the number of unsafe functions after the fix commit on average, which means programmers remove some unsafe functions when fixing vulnerabilities. However, the number of unsafe blocks before a fix commit is less than the number of unsafe blocks after a fix commits on average. The distribution of unsafe blocks shows that the width of numbers 2 to 4 is slimmer. This result is somehow unexpected and opposite to the result in function level. One explanation for this result is that in some vulnerabilities, unsafe blocks are removed; in some other vulnerabilities, programmers add unsafe blocks to fix vulnerabilities.

% \begin{table*}[t]
% \caption{Summary of descriptive statistics of safe and unsafe in different level}
% \label{tab:decript_unsafe}
% \begin{tabular}{l|llll|llll}
% \hline
% \multirow{3}{*}{Descriptive Metrics} &
%   \multicolumn{4}{c|}{Function Level} &
%   \multicolumn{4}{c}{Block Level} \\ \cline{2-9} 
%  &
%   \multicolumn{2}{c|}{Safe} &
%   \multicolumn{2}{c|}{Unsafe} &
%   \multicolumn{2}{c|}{Safe} &
%   \multicolumn{2}{c}{Unsafe} \\ \cline{2-9} 
%  &
%   \multicolumn{1}{l|}{Before fix} &
%   \multicolumn{1}{l|}{After fix} &
%   \multicolumn{1}{l|}{Before fix} &
%   After fix &
%   \multicolumn{1}{l|}{Before fix} &
%   \multicolumn{1}{l|}{After fix} &
%   \multicolumn{1}{l|}{Before fix} &
%   After fix \\ \hline
% Mean &
%   \multicolumn{1}{l|}{1.38} &
%   \multicolumn{1}{l|}{1.93} &
%   \multicolumn{1}{l|}{1.57} &
%   1.55 &
%   \multicolumn{1}{l|}{1.59} &
%   \multicolumn{1}{l|}{2.25} &
%   \multicolumn{1}{l|}{1.54} &
%   1.56 \\ \hline
% Median &
%   \multicolumn{1}{l|}{0} &
%   \multicolumn{1}{l|}{1} &
%   \multicolumn{1}{l|}{1} &
%   1 &
%   \multicolumn{1}{l|}{1} &
%   \multicolumn{1}{l|}{1} &
%   \multicolumn{1}{l|}{1} &
%   1 \\ \hline
% Min &
%   \multicolumn{1}{l|}{0} &
%   \multicolumn{1}{l|}{0} &
%   \multicolumn{1}{l|}{0} &
%   0 &
%   \multicolumn{1}{l|}{0} &
%   \multicolumn{1}{l|}{0} &
%   \multicolumn{1}{l|}{0} &
%   0 \\ \hline
% Max &
%   \multicolumn{1}{l|}{28} &
%   \multicolumn{1}{l|}{28} &
%   \multicolumn{1}{l|}{47} &
%   47 &
%   \multicolumn{1}{l|}{21} &
%   \multicolumn{1}{l|}{28} &
%   \multicolumn{1}{l|}{47} &
%   47 \\ \hline
% %Sum &
% Total &
%   \multicolumn{1}{l|}{297} &
%   \multicolumn{1}{l|}{416} &
%   \multicolumn{1}{l|}{339} &
%   335 &
%   \multicolumn{1}{l|}{333} &
%   \multicolumn{1}{l|}{487} &
%   \multicolumn{1}{l|}{343} &
%   336 \\ \hline
% \end{tabular}
% \end{table*}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{sections/fig/descriptive_data.pdf}
%   \caption{Violin plot showing the distribution of functions and blocks in code before or after fix commit}
%   \label{fig:violinPlot}
% \end{figure}

% \zy{Can we have the observations from Table~\ref{tab:decript_unsafe}?}
% \autoref{fig: SR_before} shows the distribution of safeness ratio in codes before submitting the fix commit in crates and \autoref{fig: SR_after} shows the distribution of safeness ratio in codes after submitting the fix commit in crates in detail. We observe that around 60\% safeness ratio of function level in code before the fix commit is below 0.5 and 55\% safeness ratio of block-level in code before the fix commit is below 0.5. The data indicates that around two-thirds of vulnerabilities are caused by unsafe code in the crates. The number of $SR \in [0,0.1] $ and $SR \in (0.9,1.0]$ is far more than any other bins. We could see that mixed code (i.e., both unsafe code and safe code) which leads to the vulnerability in a specific crate is rare. 
% The number of $SR \in [0,0.1] $ is greater in function level than block level, together with $SR \in (0.4,0.5] $, implies that modifications in code after the fix commit are both in the unsafe block and out the unsafe block inside the function body. 
% \par
% Comparing the results of two versions of codes, we can see that the number of $SR \in [0,0.1] $ decreased and the number of $SR \in (0.9,1.0] $ increased. One explanation for these observations is that programmers fix some vulnerabilities by removing unsafe code in the crates.
% The total number of vulnerabilities at the block level is less than vulnerabilities at the function level because traits without a body are only counted at the function level. 

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{sections/fig/safeness_ratio_before.pdf}
%   \caption{Safeness Ratio in Functions and Blocks before Fix Commit} 
%   \label{fig:SR_before}
% \end{figure}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{sections/fig/safeness_ratio_after.pdf}
%   \caption{Safeness Ratio in Functions and Blocks after Fix Commit} 
%   \label{fig:SR_after}
% \end{figure}

% \noindent\textbf{Vulnerability fix patterns.}
% \autoref{tab:clusterTransition} represents five classifications we gained from K-means when analyzing how programmers fix vulnerabilities in Rust crates. We discovered that most of the vulnerabilities (37.96\%) in safe code are fixed by changing in safe code. Programmers add unsafe code in safe code to fix the vulnerabilities only in 2.78\% code. About 13.89\% of vulnerabilities are fixed by removing some unsafe code. Programmers fix the 30.56\% vulnerabilities exactly in the unsafe code. There are 14.81\% vulnerabilities we cannot categorize them into the above four categories and we identified them as others. We could observe that programmers rarely add unsafe code to fix the vulnerabilities which lie in the safe code. However, around one-third of vulnerability in unsafe code is fixed by removing unsafe code. Programmers are likely to remove unsafe code to fix the vulnerabilities caused by the unsafe code. There are slight differences in numbers between \autoref{tab:clusterVul} and \autoref{tab:clusterTransition} because we run two K-means algorithms on different features of vulnerabilities to get better performance. 


% \begin{table}
%   \caption{Classification of code transition before and after fix commit}
%   \label{tab:clusterTransition}
%   \begin{tabular}{lcc}
%     \toprule
%     Type & \# vulnerabilities & \% \\
%     \midrule
%     Safe to Safe        & 82  & 37.96\%   \\
%     Safe to Unsafe      & 6   & 2.78\%   \\
%     Unsafe to Unsafe    & 66  & 30.56\%   \\
%     Unsafe to Safe      & 30  & 13.89\%   \\
%     Others              & 32  & 14.81\%   \\
%     Total               & 216 & 100\%   \\
%     \bottomrule
%   \end{tabular}
% \end{table}




